Consistency Learning via Decoding Path Augmentation for Transformers in Human Object Interaction Detection

Human-Object Interaction detection is a holistic visual recognition task that entails object detection as well as interaction classification. Previous works of HOI detection has been addressed by the various compositions of subset predictions, e.g., Image -> HO -> I, Image -> HI -> O. Recently, transformer based architecture for HOI has emerged, which directly predicts the HOI triplets in an end-to-end fashion (Image -> HOI). Motivated by various inference paths for HOI detection, we propose cross-path consistency learning (CPC), which is a novel end-to-end learning strategy to improve HOI detection for transformers by leveraging augmented decoding paths. CPC learning enforces all the possible predictions from permuted inference sequences to be consistent. This simple scheme makes the model learn consistent representations, thereby improving generalization without increasing model capacity. Our experiments demonstrate the effectiveness of our method, and we achieved significant improvement on V-COCO and HICO-DET compared to the baseline models. Our code is available at https://github.com/mlvlab/CPChoi.

==> 0_ Abstract/0_Abstract.tex <==
 
% VER1.Consistency regularization is widely used in many different tasks in computer vision to regularize multiple outputs. 
% This paper proposes a model agnostic training strategy using consistency regularization for Human object interaction (HOI) detection.
% Our training strategy generates multiple inference paths and, models are simultaneously learned with shared parameters.
% To train the multiple paths, we propose 1) set matched consistency regularization  2) set unmatched consistency regularization.  
% These two training strategies enable the path invariant robust training and solve the sparse annotation problem in HOI detection.
% To fully show the performance of our model,  we introduce the densely annotated HOI dataset that can accurately measure the performance. 
% Our experiment demonstrates the effectiveness of our method, and we achieved competitive performance compared to the baseline models.

% VER2.Human Object Interaction(HOI) detection dataset is not densely annotated. 
% To learn from the sparsely annotated dataset we propose a new training strategy for HOI transformers. 
% Our training strategy effectively learns semantic features that are not annotated in the dataset with path consistency learning. 
% Path consistency learning generates all possible inference paths and utilizes consistency regularization to train multiple inference paths.  
% Consistency regularization consists of 1) set matched consistency regularization for labeled data, 2) set unmatched consistency regularization for unlabeled data.  
% These two training strategies enable the path invariant robust training and solve the sparse annotation problem in HOI detection.
% To fully show the performance of our model,  we introduce the densely annotated HOI dataset that can accurately measure the performance. 
% Our experiment demonstrates the effectiveness of our method, and we achieved competitive performance compared to the baseline models.

% VER3.Human Object Interaction(HOI) detection task is identified as locating and classifying \texttt{<human,  verb, object>} triplets. 
% To predict a set of HOI triplets different inference sequence is possible. eg. HI$\rightarrow$ O, HO$\rightarrow$ I.
% Our training strategy generates possible inference paths and utilizes consistency regularization to train multiple inference paths. 
% Training multiple inference paths with consistency regularization allows paths to share knowledge between paths and improve each path's performance. 
% Also, pseudo labels can be generated from the multiple inference paths to train unlabeled data.
% Since HOI dataset has complex annotations, it is difficult or impossible to densely annotate a large-scale dataset. 
% We train the model with pseudo labels generated from multiple inference paths to effectively learn the semantic features of unlabeled data. 
% To fully show the performance of our model,  we introduce the densely annotated HOI dataset that can accurately measure the performance. 
% Our experiment demonstrates the effectiveness of our method, and we achieved competitive performance compared to the baseline models.
%In recent years, transformers become  

% ver4
% Two-stage detectors have been dominant structure of Human Object Interaction (HOI) detectors. 
% But with the merge of Transformers, End-to-End Transformer-based HOI detection models have become a State-of-the-art method.
% In this paper, we propose a training strategy that applies to Transformer-based architectures.
% To predict a set of HOI triplets different inference sequence is possible, e.g., HI$\rightarrow$ O, HO$\rightarrow$ I.
% Our training strategy augments the inference paths to generate multiple identical outputs and utilizes consistency regularization to train multiple inference paths. 
% This allows collaborative training, which results in improvement of performances to all the paths. 
% Also, we tackle the sparse annotation problem of the public HOI benchmark dataset and reconstruct conventional \text{pseudo label generation} scheme suitable for HOI Transformers. 
% We train the model with pseudo labels generated from multiple inference paths to effectively learn the semantic features of unlabeled data.
% To fully show the performance of our training strategy,  we build a new densely annotated dataset named as \texttt{Dico-DET}. 
% Our experiment demonstrates the effectiveness of our method, and we achieved competitive performance compared to the baseline models.

%new : Data Augmentation -> path augmentation / 

%Human Object Interaction (HOI) detection aims to localize both the human and an object as well as identify an interaction between them.
%Human Object Interaction (HOI) detection aims to classificate interaction between humans and object  
Human-Object Interaction (HOI) detection aims to predict triplets \texttt{<human, object, interaction>} about the visual relationships between humans and objects. 
%The individual predictions for each elements of the HOI is not independent, 
%Since the prediction of each element of \texttt{<human,  verb, object>} triplets are  highly dependent, each element can be inferred in different inference paths and their final outputs should be consistent.
The HOI triplets can be inferred by different inference paths, e.g., Image$\rightarrow$HI$\rightarrow$ O, Image$\rightarrow$HO$\rightarrow$ I. 
In this paper, we propose a widely applicable training strategy for Transformer in HOI detection called \textbf{Cross-Path Consistency Learning}. 
Our training strategy augments the decoding paths and all the augmented paths are regularized by cross-path consistency loss.
%\textbf{Decoding-Path Augmentation} to generate multiple decoding paths and all decoding paths are trained with consistency regularization, called \textbf{cross-path consistency loss}.
This encourages consistent representation without increasing the number of parameters in the baseline model and results in performance improvement to all paths.
% Additionally, we introduce new densely annotated test dataset called \textbf{Dense HICO-DET} to verify whether inferences can be made densely even when trained with sparsely annotated dataset.
% 제한된 파라미터개수로 좋은 feature을 배우고 robust minima를 찾음으로써? 더나은 일반화를 꾀한다.
% 저거 쓰면서 얻을수잇는 효과...generalization 
Our experiment demonstrates the effectiveness of our method, and we achieved significant improvement on V-COCO and HICO-DET compared to the baseline models.



==> 1_Introduction/1.1_motivation.tex <==
% transformer... 
% decomposition 
% task consistncy 

==> 3_Method/3_1_Revisit_HOI_Transformer.tex <==
\section{Method}
In this section, we \hwan{describe our novel end-to-end training strategy for transformers with \textbf{cross-path consistency} in Human-Object Interaction Detection.}  
% In this section, we introduce our novel training strategy in detail. 
%We propose  for transformers with multi-path consistency in Human-Object Interaction Detection.
The training strategy includes 1) augmenting the decoding path and 2) consistency regularization between predictions of multiple paths. % path 에 대한 설명?
\hwan{In Section~\ref{section3.1}, we explain two general types of transformer in Human-Object Interaction detection.
Then, we describe how our two training strategies, decoding-path augmentation and cross-path consistency learning, in Section~\ref{section3.2} and Section~\ref{section3.3}.}
%Our training schema augment the decoding path to generate multiple paths to train a model.
%For HOI detection, we augmented a path and generated 3 extra paths to train a model. 
%And without any extra decoders for each path, model is trained with only one set of encoder 
%The purpose of our work is augmenting a decoding path to multiple paths 
\subsection{Revisit Transformer in HOI detection}
\label{section3.1}
% hoi transformer는 크게 두가지로 나눌 수 있다.  2decoder with instance matching , 1decoder 
%This section explains single decoder and two decoder HOI transformer models in detail to show how our training strategy can be applied to both transformer-based HOI detection models.%추가함 
%Extension upon DETR, existing HOI transformers are composed of backbone CNN followed by encoder-decoder architecture of transformer.

% \hwan{HOI transformers are commonly extended upon DETR~\cite{carion2020end}, which are composed of backbone CNN followed by encoder-decoder architecture of transformer~\cite{Vaswani17transformer}.}
% The backbone CNN first extracts \textit{locally aggregated} feature  from input image $x \in \mathbb R^{H \times W \times 3}$. 
% Then, \hwan{the extracted features $X\in \R^{H'\times W'\times D}$} are passed into an encoder of which self-attention to \textit{globally} aggregate features.
% %At the decoding stage, the encoder feature map $F_{\text{enc}}\in\R^{D\times H'\times W'}$ and learnable position encoding $\text{p}\in \R^{N_q\times D_\text{p}}$ are the input of a decoder.
% \hwan{%At the decoding stage, the decoder takes encoded features $X \in \R^{D\times H'\times W'}$ and learnable positional embedding $p \in  \R^{N_q\times D_\text{p}}$ to predict the HOI triples. 
% %Here, $N_q$ number of queries are updated with self-attention and co-attention to highliht a specific information of the encoded features.

% In the decoding stage, the majority of the HOI transformers can be divided into two types; predicting HOI triplets at once~\cite{tamura2021qpic,zou2021end} or separately~\cite{kim2021hotr,chen2021reformulating}. 
% We will explain about common characteristics and differences between the single-decoder models and the two-decoder models.
% }

\hkc{
HOI transformers are commonly extended upon DETR~\cite{carion2020end}, which is composed of a CNN backbone followed by the encoder-decoder architecture of Transformer~\cite{Vaswani17transformer}. The CNN backbone first extracts \textit{locally} aggregated feature from input image $x \in \mathbb R^{H \times W \times 3}$. 
Then, the extracted feature map $X\in \R^{H'\times W'\times D}$ are passed into the encoder to \textit{globally} aggregate features via the self-attention mechanism. 

% Finally, the densely encoded features are cross-attended with object queries in the decoder layers.

% In the decoding stage, the majority of the HOI transformers can be distinguished by how the HOI triplets are predicted; predicting HOI triplets at once~\cite{tamura2021qpic,zou2021end} or seperately~\cite{kim2021hotr,chen2021reformulating}. 
% The commonalities and differences of the single-decoder and two-decoder models will be summarized shortly.
}
\jhp{In a decoding stage, learnable query embeddings $p\in \R^{N\times D}$ are fed into 6-layer decoder and updated into $e\in\R^{N\times D}$ by interacting with encoded feature map $X$ through cross-attention. Basically at the end of each layer, feed-forward networks for each HOI triplet element is attached to localize human and object regression, and predict interaction classes. 

At the training phase, Hungarian algorithm is used to match between ground truth labels and predictions from the decoder, and calculate the loss between them. 
The predictions unmatched with ground truth labels are considered as no object and interactions.  

In the localizing part, simple extention from DETR~\cite{tamura2021qpic,zou2021end} is to directly regress the box coordinates of humans and objects. This brings out the problem that human or object can be redundantly predicted with multiple query embeddings since the ground truth set is composed of HOI triplets. Other variants~\cite{kim2021hotr,chen2021reformulating} overcome this issue to construct extra branch for instance detection and use matching scheme for binding the relevant instances from instance decoder outputs in interaction decoder outputs.

}

%Number($N_q$) of queries which are learnable position encoding are updated with self-attention layers and co-attention layers to highlight a certain area of the encoder feature map $F_{enc}$.  
%기존: At the decoding stage, decoder uses learnable position embeddings $\text{p}\in \R^{N_q\times D_\text{p}}$ which are specialized to certain areas in encoded feature map $F_{enc}\in\R^{D\times H'\times W'}$ to update query by using self-attention with themselves and co-attention with feature map $F_{enc}$. 
%The variants of HOI transformer can be divided into two types whether object detection and action classification is done seperately~\cite{kim2021hotr,chen2021reformulating} or not~\cite{tamura2021qpic,zou2021end}. 
%We will briefly explain about each types of HOI transformer architecture below.

\paragraph{Single Decoder HOI Transformer.}
\hwan{The single-decoder HOI transformers~\cite{tamura2021qpic,zou2021end} directly infer HOI triplets in the decoding stage.
They extend DETR with an additional readout function for action classification in the decoder head.  
The decoding stage of single decoder models can be written as 
\begin{equation}
    \label{eq:single_dec}
    \begin{split}
        e &= {\text{Dec}}(p,\ X), 
    \end{split}
\end{equation}
where $e$ denotes the output embeddings, and $p$ denotes the learnable position encoding for the query input.
Then, the output embeddings are passed into feed-forward networks (FFN) for bounding box regression and action classification, as shown below.
\begin{equation}
    \label{eq:single_ffn}
    \begin{split}
        \hat{b}_h &= \text{FFN}_{h}\left(e\right), \\
        \hat{b}_o &= \text{FFN}_{o}\left(e\right), \\
        % \text{FFN}_\text{o}\left(e\right)  \\
        %\hat{c}_o &= \text{FFN}_\text{cls}\left(e\right) \\ 
        \hat{c}_{act} &= \text{FFN}_{act}\left(e\right),
    \end{split}
\end{equation}
where $\hat{b}_h,\hat{b}_o$ denotes predicted bounding boxes for the detected human or object, and $\hat{c}_{act}$ denotes the corresponding action logit.
The overall loss consists of binary cross entropy for multi-label action classification, softmax cross entropy for object classification, and $L_1$ and GIoU loss for regression.
}%Dimension 없애도 될듯? 동의합니다 보감합니다
% Only difference between single decoder HOI transformer and DETR is that readout function for action classification is added on decoder head. 
% Formulation for single decoder architecture can be written as:
% \begin{equation}
%     F_{\text{enc}} = f_{\text{enc}}(F_{\text{cnn}})
% \end{equation}
% \begin{equation}
%     e=f_{\text{dec}}(p, F_{\text{enc}})
% \end{equation}
%Here, $F_{\text{cnn}}\in\R^{D_{\text{cnn}}\times H' \times W'}$, $F_{\text{enc}}\in\R^{D \times H' \times W'}$, $e\in\R^{N_q\times D}$ denotes CNN backbone feature, encoder feature map and output query embeddings respectively and $\posE$ denotes learnable position encoding for input query and $f_{\text{enc}},f_{\text{dec}}$ for encoder, decoder respectively.
% Then, the output query embeddings $e$ are put into feed-forward networks $\text{FFN}_\text{h-box}:\R^{D}\rightarrow \R^4$,  $\text{FFN}_\text{o-box}:\R^{D}\rightarrow\R^4$, $\text{FFN}_\text{o-cls}:\R^{D}\rightarrow\R^{C_o}$ and $\text{FFN}_\text{a}:\R^{D}\rightarrow\R^{C_a}$ to get bounding box
% \begin{equation}
%     \hat{b}_h=\text{FFN}_\text{hum box}\left(e\right) 
% \end{equation}
% \begin{equation}
%      \hat{c}_o, \hat{b}_o=\text{FFN}_\text{obj cls}\left(e\right) , \text{FFN}_\text{obj box}\left(e\right) 
% \end{equation}
% \begin{equation}
%     \hat{c}_i=\text{FFN}_\text{act}\left(e\right)
% \end{equation}
% $$\mathcal{L}=\lambda_a\cdot\mathcal{L}_a+\lambda_{\text{obj}}\cdot\mathcal{L}_{\text{obj}}+\lambda_{\text{bbox}}\cdot\mathcal{L}_{\text{bbox}}+\lambda_{\text{GIoU}}\cdot\mathcal{L}_{\text{GIoU}}$$

\paragraph{Two Decoder HOI Transformer.} 
%%%% 포괄하는 formulation FFN 부분을 
\hwan{
Despite the simple extension of single decoder HOI transformers, its architecture poses a problem that same human or objects can be redundantly inferred from different queries.
Therefore, two-decoder HOI transformers~\cite{kim2021hotr,chen2021reformulating} include two different parallel decoders: \jhp{ one for instance detection and the other for interaction detection.}
% Each decoder predicts instance and interaction separately.
\jhp{The instance decoder, which is only responsible for object detection, is frozen during training so that the quality of object detection does not affect HOI detection.
The interaction decoder infers interactions and creates semantic information for human and object, so that each interaction is matched to the relevant human and object derived from the instance decoder.}
The output embeddings can be obtained by
\begin{equation}
    \label{eq:two_dec}
    \begin{split}
        % F_{\text{enc}} &= f_{\text{enc}}(F_{\text{cnn}}) \\
        % e_{\text{ins}} &= f_{\text{dec}}(p, F_{\text{enc}}) \\
        % e_{\text{int}} &= f_{\text{dec}}\left(\posE,F_{\text{enc}}\right).
        % \\ 
        % \text{alternative, } \\
        e_{\text{ins}} &= {\text{Dec}_\text{ins}}(p,\ X), \\
        e_{\text{int}} &= {\text{Dec}_\text{int}}(p,\ X),
    \end{split}
\end{equation}
where $e_{\text{ins}}$, $e_{\text{int}}$ denotes output embeddings of instance decoder and interaction decoder respectively. 
\jhp{For the final predictions of HOI triplets, similarity matching (dot-product for HOTR~\cite{kim2021hotr} and $L_1$ distance for AS-NET ~\cite{chen2021reformulating}) is used between projected interaction embeddings and instance embeddings to predict \texttt{human} and \texttt{object}, and multi-label classification is done for \texttt{interaction}.}
% Similar to the single-decoder models, output query embeddings passed into the FFNs to predict the final outputs :
\jhp{
Final predictions can be written as
\begin{equation}
    \label{eq:two_ffn}
    \begin{split}
        \hat{b}_h &= \text{sim}\big(\text{FFN}_{h}\left(e_{\text{ins}}\right),\text{FFN}\left(e_{\text{int}}\right)\big), \\ \hat{b}_o &= \text{sim}\big(\text{FFN}_{o}\left(e_{\text{ins}}\right),\text{FFN}\left(e_{\text{int}}\right)\big),  \\
        %\hat{c}_o &= \text{FFN}_\text{cls}\left(e_{\text{ins}}\right) \\ 
        \hat{c}_{act} &= \text{FFN}_{act}\left(e_{\text{int}}\right)
    \end{split}
\end{equation} %note 용례 볼 것 \
$\text{FFN}_h$ and $\text{FFN}_o$ are the projection networks that keep the dimensionality of the output queries consistent.

Since two decoder architectures freeze parameters related to instance detection, no regression loss is used. HOTR and AS-NET use cross-entropy and $L_1$ distance for instance prediction ($\hat{b}_h,\hat{b}_o$)  respectively, and for multi-label action classification, binary cross entropy is used.}

% Note: Since each output embedding is independent, it needs to combine the most related queries between interaction decoder and instance decoder.
% Therefore, the two-decoder add a matching loss $\mathcal L_{\text{match}}$ which is the distance between $e_{\text{ins}}$ and $e_{\text{int}}$ to the total losses.


%Also,  is added on the losses of the single-decoder models to preserve the advantage of DETR; eliminating the post-processing.
%Here, the distance function can be either cosine similarity or $L_p$ norm.
% In order to preserve the advantage of DETR; eliminating the post-processing, overall losses for two-decoder models only added matching loss $\mathcal L_{\text{match}}$ on the top of the loss functions of the single-decoder models.
}

% Path-wise Loss is a supervision loss that is applied to each path. 
% For our model to learn with multiple paths, decoders $f_{i,j}$ from different paths and stages share their parameters. 
% In other words, model parameters are trained to optimize loss of all possible decoding paths. 
% % This allows the size of the model to remain the same as the baseline model whether it is single decoder model or two decoder model. 
% Each path is trained with supervision losses of bounding box $\mathcal{L}_b$ , object class $\mathcal{L}_c$ and action class $\mathcal{L}_a$.
% Bounding box regression loss $\mathcal{L}_b$ is calculated with $L_1$ loss and $GIoU$ to regress the bounding box of human and object. 
% For $\mathcal{L}_c$ and $\mathcal{L}_a$ Cross Entropy loss and Binary Cross Entropy loss are used for object classification and multi-label action classification. 

% The reason why the instance and interaction decoder are presented separately is that in the case of a single decoder, redundant human or object box may appear in multiple output queries when directly infer box coordinates.
%Two-decoder models~\cite{kim2021hotr,chen2021reformulating} seperately infer instance and interaction and bind the two outputs. 
% \begin{equation}
%     F_{enc} = f_{enc}(F_{cnn})
% \end{equation}
% \begin{equation}
%     e_{ins}=f_{dec}\left(\posE,F_{enc}\right)  
% \end{equation}
% \begin{equation}
%     e_{int}=f_{dec}\left(\posE,F_{enc}\right)  
% \end{equation}
%To bind the two independent outputs, distance are calculated between output embeddings from instance decoder and output embeddings from interaction decoder to match with lowest distance.
% Therefore, ~\cite{kim2021hotr,chen2021reformulating} uses matching strategy by calculating the distance bewteen output embeddings from instance decoder $v^{instance}\in \R^{M_q\times D}$ and output embeddings of human $v^{interact}_\text{h}\in \R^{N_q\times D}$ and object $v^{interact}_\text{o}\in \R^{N_q\times D}$ from interaction decoder.
% $M_q$, $N_q$ are number of queries in instance decoder and interaction decoder respectively.
% All those matching embeddings are projected from output queries by using feedforward network $\text{FFN}:\R^D\rightarrow\R^D$. 
%HOTR uses cosine similarity and AS-NET uses $L_1$ distance to select the most related human and object in interaction queries from instance detection results. 
%The final output predictions can be derived as follows: 
%Output embedding $e_{ins}$, $e_{int}$ are then put into feed-forward networks to retrieve \texttt{<human, verb,  object>} triplets:
% \begin{equation}
%     \hat{b}_h=\text{FFN}_\text{hum box}\left(e_{ins})\right) 
% \end{equation}
% \begin{equation}
%      \hat{c}_o, \hat{b}_o=\text{FFN}_\text{obj cls}\left(e_{ins}\right) , \text{FFN}_\text{obj box}\left(e_{ins}\right) 
% \end{equation}
% \begin{equation}
%     \hat{c}_i=\text{FFN}_\text{act}\left(e_{int}\right)
% \end{equation}
% Like single decoder architecture, $\text{FFN}_\text{act}:\R^D\rightarrow\R^{C_a}$ is used for action classification.
% The loss function of two decoder models consist of instance-interaction matching loss on top of single decoder loss function. 
% For the instance-interaction matching loss, HOTR and AS-NET uses NCE(?) and pull-push scheme respectively, to maximize agreement between the related instance embeddings and projected interaction embeddings of human and object.
%  In the case of loss fucntion, binary cross entropy is used for multi-label action classification like single decoder method and instance-interaction matching loss for prediction of human and object. For the matching loss function, HOTR and AS-NET uses NCE(?) and pull-push scheme respectively, to bring the related instance embeddings and projected interaction embeddings of human and object close together.      
% $$F_{enc}=\mathbf{Enc}\left( I \right)$$
% $$e^{interact}=\mathbf{Dec}_{interact}\left(\{\text{p}^{interact}\},F_\text{enc}\right)$$
% $$e^{instance}=\mathbf{Dec}_{instance}\left(\{\text{p}^{instance}\},F_\text{enc}\right)$$
% \begin{itemize}
%     \item \textbf{Output}\\
% $$\text{H}=\underset{j}{\operatorname{argmax}}\left(\text{sim}\left(\text{FFN}_{\text{sub}}\left(e^{interact}\right),e^{instance}_j\right)\right)$$ 
% $$\text{O}=\underset{j}{\operatorname{argmax}}\left(\text{sim}\left(\text{FFN}_{\text{obj}}\left(e^{interact}\right),e^{instance}_j\right)\right)$$ 
% $$\text{I}=\text{FFN}_\text{act}\left(e^{interact})\right)$$
%     \item \textbf{Loss}
%     $$\mathcal{L}=\lambda_a\cdot\mathcal{L}_a+\lambda_{\text{h}}\cdot\mathcal{L}_{\text{h}}+\lambda_{\text{o}}\cdot\mathcal{L}_{\text{o}}$$
% \end{itemize}

==> 5_Conclusion/CO.tex <==
\subsection{Conclusion and Limitations}
In this paper, we introduced Cross-Path Consistency Learning, novel end-to-end training strategy for general transformer architecture using consistency regularization in Human-Object Interaction detection. 
Our learning scheme leverages inference paths of difference sequence by augmenting the decoding path and imposes their predictions to be consistent, which leads to better generalization without increasing model capacity.
In the future work, we aim to apply our learning strategy for the general task, not limited to HOI, and more diverse transformer architecture.
We 


==> 5_Conclusion/HKC.tex <==
\section{Conclusion}
We proposed Cross-Path Consistency learning for Human-Object Interaction detection. Through decoding-path augmentation, various decoder paths are generated which predict HOI instances in permuted sequences. Then, consistency regularization is applied path-wise to impose consistency in the predicted HOI triplets, enforcing the predictions to be inference-path invariant. Key techniques as parameter sharing and cross matching were introduced as well to enhance learning. 

Our method is conceptually simple, and can be applied to a wide range of transformer architectures. Also, it does not require additional model capacity nor inference time. The state-of-the-art results on V-COCO and HICO-DET supports our method's efficacy in various HOI detection tasks, and its robustness is approved through further empirical studies.

However, our work's limitation lies in the task on which our method was experimented. HOI detection being an intricate vision task, it is yet relatively minor. That is, our method's feasibility in simpler and more general vision tasks was not thoroughly discussed in our work. Future work is called for.

% 1. CPC for HOI
% 2. Deocding-Path Augmentation
% 3. CPC and Cross Matching
% 4. sota performance V-COCO and HICO-DET
% 5. Limitations : narrow application 

==> Table/Hico.tex <==
\begin{table*}[h!]
  \centering
  \footnotesize
  \begin{tabular}{l c c c c c c}
    \toprule
    \multicolumn{4}{c}{} & \multicolumn{3}{c}{\textbf{Default}} \\
    \cmidrule(r){5-7}
    Method & \hspace{12pt}Detector\hspace{12pt} & Backbone & \hspace{12pt}Extra\hspace{12pt} & \hspace{12pt}Full\hspace{12pt} & \hspace{6pt}Rare\hspace{6pt} & Non Rare\hspace{6pt} \\ \hline 
    % \rowcolor[gray]{0.85}\multicolumn{7}{l}{\textit{\textbf{Sequential HOI Detectors (Instance-centric)}}} \\ \hline
    % \multicolumn{5}{l}{\textit{Models \textbf{with} linguistic priors}} \\ \hline
    % \multicolumn{5}{l}{\textit{Models \textbf{without} linguistic priors}} \\ \hline
    % \multicolumn{1}{l|}{VSRL~\cite{gupta2015visual}} & COCO & VGG-19 & \multicolumn{1}{c|}{A+P} & 6.46 & 4.24 & 7.12  \\
    % \multicolumn{1}{l|}{HO-RCNN~\cite{chao2018learning}} & COCO & CaffeNet & \multicolumn{1}{c|}{A+S} & 7.81 & 5.37 & 8.54  \\
     \multicolumn{3}{l}{ \textit{\textbf{CNN-based HOI Detection Model}}} &  &  &  &  \\ \hline
    \multicolumn{1}{l|}{InteractNet~\cite{gkioxari2018detecting}} & COCO & R50-FPN & \multicolumn{1}{c|}{A} & 9.94 & 7.16 & 10.77  \\
    % \multicolumn{1}{l|}{Verb Embedding~\cite{xu2019learning}} & COCO & R50 & \multicolumn{1}{c|}{A+L} & 14.70 & 13.26 & 15.13  \\
    \multicolumn{1}{l|}{iCAN~\cite{gao2018ican}} & COCO & R50 & \multicolumn{1}{c|}{A+S} & 14.84 & 10.45 & 16.15  \\
    \multicolumn{1}{l|}{TIN~\cite{li2019transferable}} & COCO & R50 & \multicolumn{1}{c|}{A+S+P} & 17.03 & 13.42 & 18.11  \\
    \multicolumn{1}{l|}{RPNN~\cite{zhou2019relation}} & COCO & R50 & \multicolumn{1}{c|}{A+P} & 17.35 & 12.78 & 18.71  \\
    \multicolumn{1}{l|}{PMFNet~\cite{wan2019pose}} & COCO & R50-FPN & \multicolumn{1}{c|}{A+S+P} & 17.46 & 15.65 & 18.00  \\
    \multicolumn{1}{l|}{No-Frills HOI~\cite{gupta2019no}} & COCO & R152 & \multicolumn{1}{c|}{A+S+P} & 17.18 & 12.17 & 18.68  \\
    % \multicolumn{1}{l|}{Analogies~\cite{peyre2019detecting}} & COCO & R50-FPN & \multicolumn{1}{c|}{A+L} & 19.4 & 14.6 & 20.9  \\
    \multicolumn{1}{l|}{UnionDet~\cite{Kim2020UnionDet}} & COCO & R50-FPN & \multicolumn{1}{c|}{A} & 14.25 & 10.23 & 15.46 \\
    \multicolumn{1}{l|}{DRG~\cite{Gao2020DRG}} & COCO & R50-FPN & \multicolumn{1}{c|}{A+S+L} & 19.26 & 17.74 & 19.71  \\
    \multicolumn{1}{l|}{VCL~\cite{Hou2020VCL}} & COCO & R50 & \multicolumn{1}{c|}{A+S} & 19.43 & 16.55 & 20.29  \\
    \multicolumn{1}{l|}{FCMNet~\cite{Liu2020FCMNet}} & COCO & R50 & \multicolumn{1}{c|}{A+S+P} & 20.41	& 17.34	& 21.56  \\
    \multicolumn{1}{l|}{ACP~\cite{Kim2020ACP}} & COCO & R152 & \multicolumn{1}{c|}{A+S+P} & 20.59 & 15.92 & 21.98  \\
    \multicolumn{1}{l|}{DJ-RN~\cite{li2020detailed}} & COCO & R50 & \multicolumn{1}{c|}{A+S+V} & 21.34 & 18.53 & 22.18  \\
    \multicolumn{1}{l|}{ConsNet~\cite{Liu2020ConsNet}} & COCO & R50-FPN & \multicolumn{1}{c|}{A+S+L} & 22.15 & 17.12 & 23.65  \\
    \multicolumn{1}{l|}{PastaNet~\cite{li2020pastanet}} & COCO & R50 & \multicolumn{1}{c|}{A+S+P+L} & 22.65 & 21.17 & 23.09  \\
    \multicolumn{1}{l|}{IDN~\cite{yonglu2020idn}} & COCO & R50 & \multicolumn{1}{c|}{A+S} & 23.36 & 22.47 & 23.63  \\ 
    
    % \rowcolor[gray]{0.85}\multicolumn{7}{l}{\textit{\textbf{Parallel HOI Detectors}}} \\ \hline
    \multicolumn{1}{l|}{GPNN~\cite{qi2018learning}} & COCO & R152 & \multicolumn{1}{c|}{A} & 13.11 & 9.41 & 14.23  \\
    \multicolumn{1}{l|}{IPNet~\cite{wang2020learning}} & COCO & HourGlass104 & \multicolumn{1}{c|}{A} & 19.56 & 12.79 & 21.58 \\
    \multicolumn{1}{l|}{VSGNet~\cite{ulutan2020vsgnet}} & COCO & R152 & \multicolumn{1}{c|}{A+S} & 19.80 & 16.05 & 20.91  \\
    \multicolumn{1}{l|}{PD-Net~\cite{Xubin2020PDNet}} & COCO & R152 & \multicolumn{1}{c|}{A+S+P+L} & 20.81 & 15.90 & 22.28  \\ \hline 
    
    \rowcolor{Gray} \multicolumn{3}{l}{\textit{ \textbf{Transformer-based HOI Detection Model}}} &  &  &  &   \\ \hline
    \multicolumn{1}{l|}{HoiT~\cite{zou2021end}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & 23.46 & 16.91 & 25.41 \\
    \multicolumn{1}{l|}{AS-Net~\cite{chen2021reformulating}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & 28.87 & 24.25 & 30.25 \\
    \multicolumn{1}{l|}{CDN~\cite{zhang2021mining}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & \textbf{31.78} & \textbf{27.55} & \textbf{33.05} \\ \hline 
    \multicolumn{1}{l|}{HOTR~\cite{kim2021hotr}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & 25.10 & 17.34 & \textbf{27.42} \\
    \multicolumn{1}{l|}{HOTR+ \textbf{Ours}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & \textbf{26.16} & \textbf{22.84} & 27.15 \\
    \multicolumn{1}{l|}{QPIC~\cite{tamura2021qpic}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & 29.07 & 21.85 & 31.23 \\
    \multicolumn{1}{l|}{QPIC+ \textbf{Ours}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & \textbf{29.63} & \textbf{23.14} & \textbf{31.57} \\
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Performance comparison in HICO-DET}. For the Detector, COCO means that the detector is trained on COCO, while HICO-DET means that the detector is first trained on COCO and then fine-tuned on HICO-DET.  The each letter in Feature column stands for A: Appearance, S: Interaction Patterns (Spatial Correlations), P: Pose, L: Linguistic Priors, V: Volume.}
  \label{tab:HICO-DET role}
\end{table*}

==> Table/ablation_pathnum.tex <==
\begin{table*}[h]
    \centering
    \footnotesize
    \begin{tabular}{c  c c   c c   c c   c c}
         \toprule
         \multirow{3}{*}{\textbf{Method}} 
         &\multicolumn{2}{c}{$\paths_1$}
         &\multicolumn{2}{c}{$\paths_1+\paths_2$}
         &\multicolumn{2}{c}{$\paths_1+\paths_2+\paths_3$}
         &\multicolumn{2}{c}{$\paths_1+\paths_2+\paths_3+\paths_4$} \\
         
         \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
        & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo 
        \\ 
  
         \midrule
         
         \multirow{1}{*}{QPIC} &
         62.16 & 64.53 & 
             &   &
             &   &
             &   
         \\
         \midrule
        
         \multirow{1}{*}{HOTR} &
         59.83 & 64.90 &
         60.94 & 66.10 &
         61.42 & 66.77 &
         \textbf{61.60} & \textbf{66.84} 
         \\
         \bottomrule
    \end{tabular}
    \caption{Ablation Study on the number of augmented paths in V-COCO.}
    \label{table:abl_num}
\end{table*}

==> Table/ablation_pathnum_noS2.tex <==
\begin{table}[h]
    \centering
   
    \footnotesize
    \begin{tabular}{c c c c c}
         \toprule
         \multirow{1}{*}{\textbf{Number of Paths}} 
         &\multicolumn{1}{c}{1}
         &\multicolumn{1}{c}{2}
         &\multicolumn{1}{c}{3}
         &\multicolumn{1}{c}{4} \\
        %  &\multicolumn{1}{c}{\hspace*{10mm}$\paths_1$\hspace*{10mm}}
        %  &\multicolumn{1}{c}{\hspace*{6mm}$\paths_1+\paths_2$\hspace*{6mm}}
        %  &\multicolumn{1}{c}{\hspace*{2mm}$\paths_1+\paths_2+\paths_3$\hspace*{2mm}}
        %  &\multicolumn{1}{c}{$\paths_1+\paths_2+\paths_3+\paths_4$} \\
         
  
         \midrule
         
         \multirow{1}{*}{QPIC} &
         62.16 & 
         62.57&   
         62.71&  
         \textbf{63.11}
         \\
         \midrule
        
         \multirow{1}{*}{HOTR} &
         59.83 &  
         60.94 & 
         61.42 & 
         \textbf{61.60}  
         \\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation on the number of augmented paths}. Performance on the four cases of $\paths_1$, $\paths_1 + \paths_2$, $\paths_1 + \paths_2 + \paths_3$, and $\paths_1 + \paths_2 + \paths_3 + \paths_4$ are compared.}
    \label{table:abl_num}
\end{table}

==> Table/ablation_pathwise.tex <==
\begin{table*}[h]
    \centering
    % \caption{Ablation.}
    \footnotesize
    \begin{tabular}{c c c  c c   c c   c c   c c   c c}
         \toprule
         \multirow{3}{*}{\textbf{Method}} & 
         \multirow{3}{*}{\textit{Share Dec.}} &
         \multirow{3}{*}{$\  $\textit{CPC}$\  $}& \multicolumn{2}{c}{$\paths_1$}
         &\multicolumn{2}{c}{$\paths_2$}
         &\multicolumn{2}{c}{$\paths_3$}
         &\multicolumn{2}{c}{$\paths_4$}
         &\multicolumn{2}{c}{\textbf{\textit{Average}}} \\
         
         \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13} 
        &  &  & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo  
        \\ 
  
         \midrule
         
         \multirow{3}{*}{QPIC} & & &
         62.16 & 64.53 & 
         61.89 & 64.13 &
         61.73 & 64.17 &
         60.43 & 62.95 &
         61.55 $\pm$ 0.66 &
         63.95 $\pm$ 0.60
         \\
         & \checkmark& & 
         60.65 & 63.16 & 
         60.69 & 63.21 &
         59.88 & 62.26 & 
         58.10 & 60.37 & 
         59.83 $\pm$ 1.04 &
         62.25 $\pm$ 1.15
         \\
         & \checkmark&\checkmark & 
         \textbf{63.11} & \textbf{65.44} & 
         \textbf{63.31} & \textbf{65.84} &
         \textbf{63.12} & \textbf{65.40} &
         \textbf{63.01} & \textbf{65.30} &
         \textbf{63.18} $\pm$ 0.10${}^\dagger$ &
         \textbf{65.45} $\pm$ 0.20${}^\dagger$ \\
         \midrule
        
         \multirow{3}{*}{HOTR} & & &
         59.83 & 64.90 &
         59.49 & 64.28 &
         58.98 & 64.13 &
         58.90 & 63.82 &
         59.30 $\pm$ 0.48 & 
         64.28 $\pm$ 0.39
         \\
         & \checkmark& & 
         60.61 & 65.39 &
         60.63 & 65.35 &
         61.17 & 66.01 &
         60.61 & 65.67 & 
         60.75 $\pm$ 0.24 & 
         65.58 $\pm$ 0.26
         \\
         & \checkmark&\checkmark &
         \textbf{61.60} & \textbf{66.84} & 
         \textbf{61.48} & \textbf{66.70} &
         \textbf{61.58} & \textbf{66.76} &
         \textbf{61.63} & \textbf{66.76} &
         \textbf{61.57} $\pm$ 0.05${}^\dagger$ & 
         \textbf{66.76} $\pm$ 0.04${}^\dagger$
         \\
         \bottomrule
    \end{tabular}
    \caption{Ablation Study for path-wise and average results of all paths in V-COCO.}
    \label{table:abl}
\end{table*}

==> Table/rebuttal_r1_table_option2.tex <==

\begin{table}[!ht]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l  c c  c  c c }
         \toprule
         \multicolumn{1}{c}{} &\multicolumn{2}{c}{V-COCO}& \multicolumn{3}{c}{HICO-DET} \\
         \cmidrule(r){2-3}
         \cmidrule(r){4-6}
         Method & 
         \scone & 
         \sctwo & 
         $\  $ {Full} $\  $ & 
         {Rare} & 
         {Non-Rare   }
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        QPIC & 58.8 & 61.0 &29.07 &21.85& 31.23 \\
        QPIC + ours & \textbf{63.1} & \textbf{65.4}& \textbf{xx}&\textbf{xx} &\textbf{xx}  \\
         \midrule
         
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         HOTR& 55.2 & 64.4 & 25.10& 17.34&\textbf{27.42}  \\
         HOTR + ours& \textbf{61.6}&\textbf{66.8} &\textbf{xx} &\textbf{xx} &xx \\
         \bottomrule
    \end{tabular}
    \caption{Abstraction of table 2 and table 3 in main paper.}
    \label{table:rebuttal_comp2}
    
\end{table}



==> Table/rebuttal_r1_table_option4.tex <==

\begin{table}[!ht]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l  c c  c  c c }
         \toprule
         \multicolumn{1}{c}{} &\multicolumn{2}{c}{V-COCO}& \multicolumn{3}{c}{HICO-DET} \\
         \cmidrule(r){2-3}
         \cmidrule(r){4-6}
         Method & 
         \scone & 
         \sctwo & 
         $\  $ {Full} $\  $ & 
         {Rare} & 
         {Non-Rare   }
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        QPIC & 62.2* & 64.5* &29.07 &21.85& 31.23 \\
        QPIC + ours & \textbf{63.1} & \textbf{65.4}& \textbf{29.63}&\textbf{23.14} &\textbf{31.57}  \\
         \midrule
         
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         HOTR& 59.8* & 64.9* & 25.10& 17.34&\textbf{27.42}  \\
         HOTR + ours& \textbf{61.6}&\textbf{66.8} &\textbf{26.16} &\textbf{22.84} &27.15  \\
         \bottomrule
    \end{tabular}
    \caption{Table 1 in main paper.}
    \label{table:rebuttal_comp4}
    
\end{table}



==> Table/rebuttal_r3_qpicfreezeenc.tex <==

\begin{table}[h]
    \centering
    % \caption{Ablation.}
    \footnotesize
    % \small
    \captionsetup{aboveskip=2pt}
    \begin{tabular}{c c  c  c}
         \toprule
          
        %  \multirow{1}{*}{\textit{Freeze Enc.}} &
         \multirow{1}{*}{\textit{Share Dec.}} &
         \multirow{1}{*}{$\  $\textit{CPC}$\  $}& 
         \multirow{1}{*}{\textbf{QPIC} ($\mathcal{P}_1$)} &
        
         \multirow{1}{*}{\textbf{HOTR} ($\mathcal{P}_1$)} 
         
         \\
         
         \midrule    
      
         
      
         
         
         \checkmark &\checkmark &
         \textbf{65.0} \color{blue}(+1.4)&\textbf{61.6 } \color{blue}(+1.8) \\
         
        
          &\checkmark & 
         64.1 \color{blue}(+0.5) & 61.2 \color{blue}(+1.4) \\
         
        
         \checkmark  & &
         64.0 \color{blue}(+0.4)&60.6 \color{blue}(+0.8)
         \\
         
           & &
         63.6 \color{blue}(+0.0)&59.8 \color{blue}(+0.0)
         \\
         
        
         
         \bottomrule
    \end{tabular}
    \caption{
    % Path-wise and average results on V-COCO. 
    Ablations for decoder sharing and CPC in $\mathcal{P}_1$.}
    \label{table:abl_rebuttal}
\end{table}

% \begin{table}[h]
%     \centering
%     % \caption{Ablation.}
%     \footnotesize
%     % \small
%     \begin{tabular}{c  c   c c }
%          \toprule
%          \multirow{1}{*}{\textbf{Method}} & 
%         %  \multirow{1}{*}{\textit{Freeze Enc.}} &
%          \multirow{1}{*}{\textit{Share Dec.}} &
%          \multirow{1}{*}{$\  $\textit{CPC}$\  $}& \multicolumn{1}{c}{$\paths_1$}
         
%          \\
         
%          \midrule    
%          \midrule
         
%          \multirow{4}{*}{QPIC} 
         
         
%          &\checkmark &\checkmark &
%          \textbf{65.0}  \\
         
        
%          & &\checkmark &
%          64.1  \\
         
        
%          &\checkmark  & &
%          64.0 
%          \\
         
%          &  & &
%          63.6
%          \\
         
%          \midrule
         
         
        
%          \multirow{4}{*}{HOTR} 
         
         
%          &\checkmark & \checkmark&
%          \textbf{61.6} 
%          \\
         
         
%          &&\checkmark  &
%          61.2 
%          \\
         
%          & \checkmark& &
%          60.6 
%          \\
%          & & &
%          59.8 
%          \\
         
         
%          \bottomrule
%     \end{tabular}
%     \caption{
%     % Path-wise and average results on V-COCO. 
%     Ablations for decoder sharing and CPC in $\mathcal{P}_1$.}
%     \label{table:abl_rebuttal}
% \end{table}


==> Table/supple_asnet.tex <==

\begin{table}[!h]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l c c   c  c c }
         \toprule
         \multicolumn{1}{c}{} &
         \multicolumn{2}{c}{} &
         \multicolumn{3}{c}{HICO-DET} \\

         \cmidrule(r){4-6}
         Method & 
         epoch &
         $\lambda$&
         $\  $ {Full} $\  $ & 
         {Rare} & 
         {Non-Rare   }
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         AS-Net&90&-&28.87& 24.25&30.25\\
         AS-Net + ours&90&0.5&\textbf{29.13}&\textbf{25.18} &\textbf{30.31}  \\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison of our training strategy with AS-Net on HICO-DET}. 
    }
    \label{table:supple_asnet}
    
\end{table}


==> Table/supple_coef_hotr.tex <==
\begin{table}[!h]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l  c c  c }
         \toprule

    
         Dataset 
         & epoch
         & $\lambda$ 
         & $t_\text{max}$
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        V-COCO 
        & 90
        & 1
        & 30\\
       
         \midrule
         
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         HICO-DET
        & 50
        & 0.2
        & 20\\
         \bottomrule
    \end{tabular}
    %\caption{\textbf{Hyperparameters for the weight scheduler for HOTR}}
    % \caption{\textbf{Weight scheduler for total CPC loss for HOTR}}
    \caption{\textbf{Weight scheduler settings for HOTR}}
    % \caption{\textbf{Total CPC loss coefficient for HOTR}}
    \label{table:hotr-coef}
    
\end{table}

==> Table/supple_coef_qpic.tex <==
\begin{table}[!h]
    \centering
    \footnotesize
    % \caption{Ablation.}

    \begin{tabular}{l  c c  c }
         \toprule

    
         Dataset 
         &epoch
         & $\lambda$ 
         & $t_\text{max}$
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        V-COCO 
        & 90
        & 0.2
        & 30\\
       
         \midrule
         
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         HICO-DET
        & 90
        & 0.2
        & 30\\
         \bottomrule
    \end{tabular}
    %\caption{\textbf{Total CPC loss coefficient for QPIC}}
    \caption{\textbf{Weight scheduler settings for QPIC}}
    \label{table:qpic-coef}
    
\end{table}

==> Table/supple_hoit.tex <==
% \begin{table}[!h]
%     \centering
%     \footnotesize
%     % \caption{Ablation.}
    
%     \begin{tabular}{l c c   c   }
%          \toprule
%          \multicolumn{1}{c}{} &
%          \multicolumn{2}{c}{} &
%          \multicolumn{3}{c}{V-COCO} \\

%          \cmidrule(r){4}
%          Method & 
%          epoch &
%          $\lambda$&
%          $\scone $ & 
%          \\
%          \midrule
%          \midrule
         
%         %  \rowcolor{Gray} 
%         %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
%         %  \\ \midrule
        
%         %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
%         HoiT & 150 & & 48.75* &  \\
%         HoiT + ours & 150 & 0.2 &49.34& \\
%          \bottomrule
%     \end{tabular}
%     \caption{\textbf{Comparison of our training strategy with HoiT on V-COCO and HICO-DET}. 
%     * signifies our results reproduced with the official implementation codes of ~\cite{HOITR}.}
    
%     \label{table:supple_hoit}
    
% \end{table}

\begin{table}[!h]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l c c   l}
         \toprule
         \multicolumn{1}{c}{} &
        %  \multicolumn{2}{c}{} &
         \multicolumn{3}{c}{V-COCO} \\
         \cmidrule(l){2-4}
         Method & 
         epoch &
         $\lambda$&
         \scone 
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
          HoiT&150&-&48.75*\\
         HoiT + ours&150&0.2&\textbf{49.34} \\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison of our training strategy with HoiT on V-COCO}. * signifies our results reproduced with the official implementation codes of~\cite{HOITR}. 
    }
    \label{table:supple_hoit}
    
\end{table}


==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/0_ Abstract/0_Abstract.tex <==
 
% VER1.Consistency regularization is widely used in many different tasks in computer vision to regularize multiple outputs. 
% This paper proposes a model agnostic training strategy using consistency regularization for Human object interaction (HOI) detection.
% Our training strategy generates multiple inference paths and, models are simultaneously learned with shared parameters.
% To train the multiple paths, we propose 1) set matched consistency regularization  2) set unmatched consistency regularization.  
% These two training strategies enable the path invariant robust training and solve the sparse annotation problem in HOI detection.
% To fully show the performance of our model,  we introduce the densely annotated HOI dataset that can accurately measure the performance. 
% Our experiment demonstrates the effectiveness of our method, and we achieved competitive performance compared to the baseline models.

% VER2.Human Object Interaction(HOI) detection dataset is not densely annotated. 
% To learn from the sparsely annotated dataset we propose a new training strategy for HOI transformers. 
% Our training strategy effectively learns semantic features that are not annotated in the dataset with path consistency learning. 
% Path consistency learning generates all possible inference paths and utilizes consistency regularization to train multiple inference paths.  
% Consistency regularization consists of 1) set matched consistency regularization for labeled data, 2) set unmatched consistency regularization for unlabeled data.  
% These two training strategies enable the path invariant robust training and solve the sparse annotation problem in HOI detection.
% To fully show the performance of our model,  we introduce the densely annotated HOI dataset that can accurately measure the performance. 
% Our experiment demonstrates the effectiveness of our method, and we achieved competitive performance compared to the baseline models.

% VER3.Human Object Interaction(HOI) detection task is identified as locating and classifying \texttt{<human,  verb, object>} triplets. 
% To predict a set of HOI triplets different inference sequence is possible. eg. HI$\rightarrow$ O, HO$\rightarrow$ I.
% Our training strategy generates possible inference paths and utilizes consistency regularization to train multiple inference paths. 
% Training multiple inference paths with consistency regularization allows paths to share knowledge between paths and improve each path's performance. 
% Also, pseudo labels can be generated from the multiple inference paths to train unlabeled data.
% Since HOI dataset has complex annotations, it is difficult or impossible to densely annotate a large-scale dataset. 
% We train the model with pseudo labels generated from multiple inference paths to effectively learn the semantic features of unlabeled data. 
% To fully show the performance of our model,  we introduce the densely annotated HOI dataset that can accurately measure the performance. 
% Our experiment demonstrates the effectiveness of our method, and we achieved competitive performance compared to the baseline models.
%In recent years, transformers become  

% ver4
% Two-stage detectors have been dominant structure of Human Object Interaction (HOI) detectors. 
% But with the merge of Transformers, End-to-End Transformer-based HOI detection models have become a State-of-the-art method.
% In this paper, we propose a training strategy that applies to Transformer-based architectures.
% To predict a set of HOI triplets different inference sequence is possible, e.g., HI$\rightarrow$ O, HO$\rightarrow$ I.
% Our training strategy augments the inference paths to generate multiple identical outputs and utilizes consistency regularization to train multiple inference paths. 
% This allows collaborative training, which results in improvement of performances to all the paths. 
% Also, we tackle the sparse annotation problem of the public HOI benchmark dataset and reconstruct conventional \text{pseudo label generation} scheme suitable for HOI Transformers. 
% We train the model with pseudo labels generated from multiple inference paths to effectively learn the semantic features of unlabeled data.
% To fully show the performance of our training strategy,  we build a new densely annotated dataset named as \texttt{Dico-DET}. 
% Our experiment demonstrates the effectiveness of our method, and we achieved competitive performance compared to the baseline models.

%new : Data Augmentation -> path augmentation / 

%Human Object Interaction (HOI) detection aims to localize both the human and an object as well as identify an interaction between them.
%Human Object Interaction (HOI) detection aims to classificate interaction between humans and object  
Human-Object Interaction (HOI) detection aims to predict triplets \texttt{<human, object, interaction>} about the visual relationships between humans and objects. 
%The individual predictions for each elements of the HOI is not independent, 
%Since the prediction of each element of \texttt{<human,  verb, object>} triplets are  highly dependent, each element can be inferred in different inference paths and their final outputs should be consistent.
The HOI triplets can be inferred by different inference paths, e.g., Image$\rightarrow$HI$\rightarrow$ O, Image$\rightarrow$HO$\rightarrow$ I. 
In this paper, we propose a widely applicable training strategy for Transformer in HOI detection called \textbf{Cross-Path Consistency Learning}. 
Our training strategy augments the decoding paths and all the augmented paths are regularized by cross-path consistency loss.
%\textbf{Decoding-Path Augmentation} to generate multiple decoding paths and all decoding paths are trained with consistency regularization, called \textbf{cross-path consistency loss}.
This encourages consistent representation without increasing the number of parameters in the baseline model and results in performance improvement to all paths.
% Additionally, we introduce new densely annotated test dataset called \textbf{Dense HICO-DET} to verify whether inferences can be made densely even when trained with sparsely annotated dataset.
% 제한된 파라미터개수로 좋은 feature을 배우고 robust minima를 찾음으로써? 더나은 일반화를 꾀한다.
% 저거 쓰면서 얻을수잇는 효과...generalization 
Our experiment demonstrates the effectiveness of our method, and we achieved significant improvement on V-COCO and HICO-DET compared to the baseline models.



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/0_ Abstract/0_ab.tex <==
% Previous methods for Human-Object Interaction Detection
% use subset of prediction for inference or auxiliary ways,
% \eg, specify interaction after H-O pair or using instance interactiveness for post-processing. 
% Recently, transformer based architecture for HOI has emerged, breaking down the existing 2-stage methods in an end-to-end manner.
% By leveraging both concepts, we propose novel end-to-end cross path consistency learning for transformer in HOI detection. 
% The proposed method enforces all the possible predictions from permuted inference sequences to be consistent. 
% This simple scheme makes the model to learn consistent representation, thus improves generalization without increasing model capacity. 
% Our experiment demonstrates the effectiveness of our method, and we achieved significant improvement on V-COCO and HICO-DET compared to the baseline models.
Human-Object Interaction detection is a holistic visual recognition task that entails object detection as well as interaction classification.
% Subsets of predictions \texttt{<Human, Object, Interaction>} are commonly used in auxiliary ways for Human-Object Interaction (HOI) detection,
% \eg predicting \texttt{<Human, Interaction>} as auxiliary output, to help predict HOI triplets
Previous works of HOI detection has been addressed by the various compositions of subset predictions, \eg, Image $\rightarrow$ HO $\rightarrow$ I, Image $\rightarrow$ HI $\rightarrow$ O.
% \texttt{<Human, Object>}$\rightarrow$ \texttt{<Interaction>}, \texttt{<Human, Interaction>}$\rightarrow$ \texttt{<Object>}.
% triplets \texttt{<Human, Object, Interaction>} were 
Recently, transformer based architecture for HOI has emerged, which directly predicts the HOI triplets in an end-to-end fashion (Image $\rightarrow$ HOI).  
%By leveraging both concepts, we propose a novel end-to-end \textbf{cross path consistency learning} method for transformer in HOI detection. 
Motivated by various inference paths for HOI detection, 
we propose cross-path consistency learning (CPC), which is a novel end-to-end learning strategy to improve HOI detection for transformers by leveraging augmented decoding paths.
CPC learning enforces all the possible predictions from permuted inference sequences to be consistent. 
This simple scheme makes the model learn consistent representations, thereby improving generalization without increasing model capacity.
Our experiments demonstrate the effectiveness of our method, and we achieved significant improvement on V-COCO and HICO-DET compared to the baseline models. 
Our code is available at \href{https://github.com/mlvlab/CPChoi}{https://github.com/mlvlab/CPChoi}.
% \footnote{Our code is available at \href{https://github.com/jihwanp/cpcHOI}{https://github.com/jihwanp/cpcHOI}}
\vspace{-3mm}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/1_Introduction/1.1_motivation.tex <==
% transformer... 
% decomposition 
% task consistncy 

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/1_Introduction/1_Introduction.tex <==
\label{sec:intro}
\section{Introduction}

Human-Object Interaction (HOI) detection is a holistic visual recognition task that includes detecting individual objects as \texttt{<human, object>}, while properly classifying the type of \texttt{<interaction>}. % set prediction 
Previous HOI detectors~\cite{gkioxari2018detecting,wang2020learning,li2020pastanet,ulutan2020vsgnet} were mainly built on object detection models. 
They commonly extend CNN-based object detectors~\cite{ren2016faster,lin2017feature,newell2016stacked} with an additional head for interaction classification, \eg, humans and objects are detected first, and their interaction is associated subsequently.

To alleviate the high computation cost of such two-stage HOI detection methods, one-stage models~\cite{wang2020learning,Kim2020UnionDet,liao2019ppdm} have been proposed for faster detection.
These models perform interaction prediction and object detection in parallel.
They compensate for their lower performance with auxiliary predictions for the HOI subsets, \ie, auxiliary predictions for subset \texttt{<human, interaction>} or \texttt{<object, interaction>} may help HOI prediction through post-processing.
However, these works demand different network architectures for each auxiliary prediction, due to strict disciplines for each network's input.
Hence, to introduce flexibility, transformer-based architectures~\cite{kim2021hotr, tamura2021qpic, chen2021reformulating, touvron2021training} have recently been adopted for HOI detection. 
% Based on the recent success of the transformer architecture in the vision area, HOI detections with transformer have been proposed
They reformulate the HOI detection problem as a direct set prediction building on  DETR~\cite{carion2020end}.


\input{Figure_caption/figure1}
% Motivated by the HOI detection methods that leverage the subset predictions and transformer architecture, 
Motivated by various inference paths in HOI detectors, we propose a simple yet effective method to train HOI transformers. 
% we propose a simple yet effective method to train HOI transformers with subset predictions auxiliary predictions. 
%The main branch that directly decodes the input feature to HOI triplets, 
We augment the decoding paths with respect to the possible prediction sequences of HOI triplets.  
% In contrast to CNN-based HOI detectors, HOI transformers deal with its intermediate features as feature embeddings. 
% It leads to the decoding stage that can decode the input query repeatedly by the attention mechanism of the decoder.  
% Therefore, transformers no need to be added an additional parameter to decode the new format of the auxiliary output. 
Then, with the cascade structure of transformers, an input query is sequentially decoded into auxiliary sub-task outputs and the final output.
% With the help of the transformer architecture, an input query can be sequentially decoded into an auxiliary output as well as the final output in a cascaded manner.
The stage of each augmented paths stage shares a decoder, in a multi-task learning fashion. 
We further improve our method to leverage the augmented decoding paths by enforcing the outputs from the various paths to be consistent. 
% With the decoding path augmentation, we further expand each path to benefit each other. 
% From the perspective of HOI instance prediction, outputs from the HOI transformers should be consistent regardless of their decoding paths. 
Accordingly, we propose \textbf{Cross-Path Consistency (CPC) Learning}, which aims to predict HOI triplets regardless of inference sequences.
% Previous works of HOI detection only utilize the auxiliary prediction as a calibration score. 
% In other words, each independently predicted score of the different subset of HOI is only gathered in the post-processing and cannot be transported to the end-to-end pipeline.
% In contrast, we present novel cross-path-consistency regularization between each output in the training phase.

% Similar to cross-\textit{task} consistency~\cite{zamir2020robust}, cross-\textit{path} consistency retains inference path invariance. 
% % is a kind of in-training model ensemble 
% In cross-path consistency learning (Fig.~\ref{fig:consistency variants}(c)), the main task $\mathcal{Y}$ (\eg, Image$\rightarrow$HOI) is disentangled into task subsets $\mathcal{Y}_s$ and $\mathcal{Y}-\mathcal{Y}_s$ (\eg, Image$\rightarrow$HO$\rightarrow$I).
% The main task function $f_{\mathcal{X}\mathcal{Y}}$ is trained by enforcing its output and the composition of sub-task predictions from the cascade architecture, to be consistent.
% % Our cross-path consistency resembles an ensemble learning method that is temporarily adopted only while training.
% Our cross-path consistency method is temporarily adopted only while training whereas cross-\textit{task} consistency requires extra networks for each auxiliary task.  

%%%%%%%
Similar to cross-\textit{task} consistency~\cite{zamir2020robust}, cross-\textit{path} consistency retains \textit{inference path invariance}. 
However, cross-path consistency learning does not require additional pre-trained networks. 
In contrast to cross-task consistency, which demands an auxiliary network to train the main task $\mathcal{X} \rightarrow \mathcal{Y}$ (Figure~\ref{fig:consistency variants}-(b)), cross-path consistency defines an auxiliary domain $\mathcal{Y}_s$ in between $\mathcal{X}$ and $\mathcal{Y}$ (Figure~\ref{fig:consistency variants}-(c)).
%The difference is that cross-path consistency learning does not require additional pre-trained networks. Compared to cross-task consistency learning that adopts an auxiliary network to train main task $\mathcal{X} \rightarrow \mathcal{Y}$ (Figure~\ref{fig:consistency variants}(b)), cross-path consistency defines a sub-task Image $\mathcal{Y}_s$ in between $\mathcal{X}$ and $\mathcal{Y}$ (Figure~\ref{fig:consistency variants}(c)). 
In other words, the main task $\mathcal{X} \rightarrow \mathcal{Y}$ (\ie, Image$\rightarrow$HOI) is divided into subtasks $\mathcal{X} \rightarrow \mathcal{Y}_s$ and $\mathcal{Y}_s \rightarrow \mathcal{Y}$ (\eg, Image$\rightarrow$HO$\rightarrow$I).
The main task function $f_{\mathcal{X}\mathcal{Y}}$ is then trained by enforcing its output and the composition of sub-task predictions to be consistent.
Moreover, cross-path consistency learning is temporarily adopted for training only.
%%%%%%%%




Our training strategy can be generalized to any transformer based architecture, and can be applied in an end-to-end method.
Extensive experiments show that HOI transformers trained with CPC learning strategy achieves substantial improvements in two popular HOI detection benchmarks: V-COCO and HICO-DET. 
The contribution of this work can be \jhprev{summarized as the followings}:
% Our training strategy is transformer-based model agnostic learning scheme with an end-to-end fashion and we confirm that it achieves promising results in two popular HOI detection benchmarks: V-COCO and HICO-DET. The contribution of this work can be summarized as the followings:
\begin{itemize}
    % submission version
    % \item We propose \textbf{Cross-Path Consistency} (CPC) learning, which is a novel end-to-end learning strategy to improve transformers for HOI detection leveraging various inference paths. 
    % % \item We propose a novel end-to-end \textbf{Cross-Path Consistency Learning} for HOI detection. Our method is agnostic to transformer architectures.
    % \item We propose \textbf{Decoding-Path Augmentation} to generate various inference paths which are compositions of subtasks with a shared decoder for effective training. 
    \jhprev{
    \item We propose \textbf{Cross-Path Consistency} (CPC) learning, which is a novel end-to-end learning strategy to improve transformers for HOI detection leveraging various inference paths. 
    % \item We propose a novel end-to-end \textbf{Cross-Path Consistency Learning} for HOI detection. Our method is agnostic to transformer architectures.
    In this learning scheme, we use \textbf{Decoding-Path Augmentation} to generate various inference paths which are compositions of subtasks with a shared decoder for effective training.  
    % Additionally, \textbf{Cross Matching} is used to give instructions on which output to be consistent.
    }
    % , and a \textbf{Cross Matching} scheme to bind predictions from different paths. 
    \item Our training scheme achieves substantial improvements on V-COCO and HICO-DET without increasing \textit{model capacity} and \textit{inference time}.  
    % before submission
    % \item We propose Cross-Path Consistency Learning on transformer-based architectures for HOI detection. This learning scheme is applicable regardless of transformer variants, and is performed in an end-to-end manner.
    % \item We propose two training techniques for consistency learning: Decoding Path Augmentation to infer different semantic information in a single decoder, and the Cross Matching scheme to bind identical semantic predictions for consistency learning. 
    % \item Our training scheme achieves better performance compared to baseline models in V-COCO and HICO-DET without increasing model capacity and inference time.  
\end{itemize}



% \subsection{Motivation}
% \jhp{- Different from DJ-RN? : multi modality vs single consistency

% - 000 Robust learning through consistency : \text{inference path invariance}

% training consistency learning from scratch with multi-bipartite matching(?)
% }
% \subsection{Contribution}
% \jhp{
% - propose novel(?) training scheme for HOI transformer using multi-path output consistency with no additional inference time

% - query modifier(?)
% }

% Motivation 
% - DJ-RN과 다른점? single modality
% - robust learning cross task consistency 의 keyword가져감: inference path invariance
%  다른점? function composition vs query composition (ours)
% Contribution
% - single modaliry에서 HOI transformer의 multi-path output consistency training scheme제안 (with no additional inference time) 
% - multi-path를 하나의 shared decoder로 efficient하게 training하기위한 query modifier제안

% \begin{figure}[tp] \centering
% \includegraphics[width=300pt]{Figure/consistency.png} \caption{Variants of consistency learning. } \label{fig:consistency variants} \end{figure}
% \usepackage{subcaption}



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/2_Related works/2_1_HOI.tex <==
\section{Related Works}
\subsection{Human Object Interaction Detection}
\label{section2.1}
Human-Object Interaction (HOI) detection has been proposed in ~\cite{gupta2015visual}.
Later, human-object detectors have been improved using human or instance appearance and their spatial relationship~\cite{gkioxari2018detecting, kolesnikov2018detecting, gao2018ican}.
%Especially, InteractNet~\cite{gkioxari2018detecting} extended an existing object detector by introducing an action-specific density map to localize target objects based on the appearance of a detected human.
%Note that interaction detection based on visual cues from individual boxes often suffers from the lack of contextual information.
%So iCAN~\cite{gao2018ican} proposed an instance-centric attention module that extracts contextual features complementary to the features from the localized objects/humans.
On the other hand, graph-based approaches~\cite{qi2018learning, ulutan2020vsgnet, Gao2020DRG, Wang2020Hetero} have been proposed to clarify the action between the \texttt{<human,  object>} pair.
%GPNN~\cite{qi2018learning}, VSGNet~\cite{ulutan2020vsgnet} and DRG~\cite{Gao2020DRG}  proposes graph-based HOI recognition~\cite{Wang2020Hetero}---a general framework that explicitly represents HOI structures with graphs and automatically infers the optimal graph structures.
%Deep Contextual Attention~\cite{Wang2019deepcontext} leverages contextual information by a contextual attention framework in HOI.
% External

HOI detection models based on only visual cues often suffer from the lack of contextual information. 
Thus, recent works utilize external knowledge to improve the quality of HOI detection.
%Since the performance of HOI detection is dependent on how well we recognize the appearance of human actions, 
Human pose information extracted from external models~\cite{cao2017realtime,chen2018cascaded,he2017mask, li2019crowdpose} or linguistic priors and knowledge graph models show meaningful improvement in performance~\cite{zhou2019relation, Liu2020FCMNet, peyre2018detecting,xu2019learning,gupta2017aligned,gkanatsios2019deeply,li2020pastanet, Xubin2020PDNet, Liu2020ConsNet}.
%Interactiveness Knowledge has also been implemented in previous works~\cite{li2019transferable} by adding an additional inference stage where the model learns the probability of interactiveness by combining multiple HOI training datasets.
%Pose estimation information~\cite{wan2019pose,li2019crowdpose} is used to further extract features from the human region.
%Mask R-CNN is used to parse the human body parts and form a graph that connects each body part with target objects~\cite{zhou2019relation, Liu2020FCMNet, li2020pastanet}.
%In another, linguistic priors and knowledge graphs have also been used to improve HOI detection by compensating for the rare triplets on the dataset. ~\cite{peyre2018detecting,xu2019learning,gupta2017aligned,gkanatsios2019deeply,li2020pastanet, Xubin2020PDNet, Liu2020ConsNet}.
%Functional Generalization~\cite{bansal2019detecting} uses word embedding with image features to define a set of objects that have similar \textit{functions}, and trains the HOI model by interchanging functionally similar objects.

Since the majority of the previous works are based on two-stage methods with slower inference time, attempts for faster HOI detection by introducing simple end-to-end multi-layer perceptrons~\cite{gupta2019no}, or directly detecting interaction points~\cite{wang2020learning,liao2019ppdm}, or union regions~\cite{Kim2020UnionDet, Hou2020VCL, yonglu2020idn} have been suggested. 

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/2_Related works/2_2_Vision_Transformer.tex <==
\subsection{Transformers in Computer Vision}
\label{section2.2}
Transformer has become the state-of-the-art method in many computer vision tasks. 
In image classification, ~\cite{dosovitskiy2020image} has shown competitive performance on ImageNet without any convolution layers.
DeiT~\cite{touvron2021training} applied knowledge distillation to data-efficiently train the vision transformer.
To extract multi-scale image features, Swin Transformer~\cite{Liu_2021_ICCV} proposed shifted window based self-attention modules that effectively aggregate small patches to increase the receptive field.
In the object detection task, DETR~\cite{carion2020end} has proposed an end-to-end framework eliminating the need for hand-designed components.
DETR's bipartite matching loss between the predicted set and the ground truth labels enables direct set prediction at inference.
Recently, DETR's late convergence problem has been tackled in~\cite{zhu2020deformable,meng2021conditional,Gao_2021_ICCV}.

Inspired by DETR, transformer-based  HOI (Human-Object Interaction)  detectors~\cite{kim2021hotr,tamura2021qpic,chen2021reformulating,zou2021end,dong2021visual} have been recently proposed. 
HOI transformer models have two types of structure, one decoder model and the two decoder model.
The one-decoder model which follows the structure of DETR~\cite{carion2020end} predicts  triplets from the output of a single decoder. 
QPIC~\cite{tamura2021qpic} and HoiT~\cite{zou2021end} are one-decoder models that output \texttt{<human, object, interaction>} triplets directly with multiple interaction detection heads. 
Two-decoder models use two transformer decoders to output distinctive targets. %%%%의미 더쓰기.  %???%%.
For instance, HOTR~\cite{kim2021hotr} and AS-NET~\cite{chen2021reformulating} are composed of an instance decoder that outputs object and an interaction decoder that outputs interaction. 
% To bind the outputs of two decoders, HOTR suggested adopting an HO-pointer that makes use of similarity between two different decoder outputs. In the case of AS-NET, the Semantic Embedding that push and pull the two outputs was introduced. 
%two decoder vs one decoder 장단점..
In contrast to previous works that are trained with a single inference path, our model learns with the augmented decoding paths. 
% the help of multiple inference paths generated by Decoding-Path Augmentation.
% any???
Also, our framework can be applied to any transformer-based model. 
% with no additional computation time.
More explanation of HOI transformers are in Section~\ref{section3.1}.
% two stage 채우기 



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/2_Related works/2_3_Consistency_learning.tex <==
\subsection{Consistency Learning in Vision}
\label{section2.3}
Consistency constraints applied to many computer vision topics have been extensively studied.
% There are extensive works in consistency constraints that extend to many different topics in computer vision. 
In semi-supervised learning, consistency regularization is widely used to train the model to be invariant to input noise.
Label consistency methods~\cite{laine2016temporal,xie2020unsupervised,miyato2018virtual,tarvainen2017mean} augment or perturb an input image and apply consistency loss between model predictions.  
CDS~\cite{NEURIPS2019_d0f4dae8} explored object detection in a semi-supervised setting with classification and localization consistency regularization. 
Also, consistency regularization in cyclic form is commonly used in generative models~\cite{zhu2017unpaired}, image matching~\cite{7298723,zhou2016learning}, temporal correspondence~\cite{dwibedi2019temporal}, and in many other domains. 

% Our consistency training schema is most relevant to cross-task consistency learning~\cite{zamir2020robust}.
% Cross-task consistency learning is based on inference-path invariance, where consistency loss is applied to paths with the same end point but with different intermediate domains.
% For instance, if $f_{\mathcal{X}\mathcal{Y}}(x)$ is a neural network that receives $x$ as input and outputs domain $y$, output of $f_{\mathcal{Y}\mathcal{Y}_a}\circ f_{\mathcal{X}\mathcal{Y}}(x)$ should be consistent with the output of $f_{\mathcal{Y}\mathcal{Y}_a}(y)$.
% %%%%%% 다른점 강조 더하기
% Different from cross-\textit{task} consistency, our cross-\textit{path} consistency learning does not require pre-trained models for each inference paths to impose consistency between them.
% % Also, we augment the decoding path with intermediate output $y_s$ before final output where task consistency learning extends to another domain $y_a$ after the target domain.
% Also, as shown in Figure~\ref{fig:consistency variants}, cross-task consistency uses auxiliary task $\mathcal{Y}_a$ which is extended from the target output to train the main task function $f_{\mathcal{X}\mathcal{Y}}$, whereas cross-path consistency augments the inference path with intermediate output $\mathcal{Y}_s$ to impose consistency across all paths. 
% Details on augmenting decoding paths is described in section~\ref{section3.2} 
% multiple sequence of thought 이거 뭐라고 할까.. 
% 더써야되면 2.2에 Cycle consistency 류들 쓰기.. 

\paragraph{Comparison with Consistency Learning}
Our consistency training scheme is relevant to cross-task consistency learning~\cite{zamir2020robust}.
Cross-task consistency learning is based on inference-path invariance, where the predictions should be consistent regardless of the inference paths.

% It uses auxiliary task $\mathcal{Y}_a$ as a target of objective function for consistency to train main task function $f_{\mathcal{X}\mathcal{Y}}$ where as our cross-path consistency train main task function $f_{xy}$ by using disentangled task $y_s$ as intermediate output and cascaded form of augmented path to make main task output $y$ to be consistent.


As shown in Figure~\ref{fig:consistency variants} (b), cross-\textit{task} consistency learning uses an auxiliary task $\mathcal{Y}\rightarrow \mathcal{Y}_a$ to train the main task function $f_{\mathcal{X}\mathcal{Y}}$, 
\ie, given $x$ from the query domain, and $y$ from target domain $\mathcal{Y}$, predictions of $f_{\mathcal{Y}\mathcal{Y}_a}\circ f_{\mathcal{X}\mathcal{Y}}(x)$ and $f_{\mathcal{Y}\mathcal{Y}_a}(y)$ are expected to be consistent.
% \ie, given $x$ and $y$ as datapoint from query domain and task $\mathcal{Y}$ respectively, consistent predictions between $f_{\mathcal{Y}\mathcal{Y}_a}\circ f_{\mathcal{X}\mathcal{Y}}(x)$ and $f_{\mathcal{Y}\mathcal{Y}_a}(y)$ are expected.
Different from cross-\textit{task} consistency, our cross-\textit{path} consistency learning (Figure~\ref{fig:consistency variants} (c)) trains the main task function $f_{\mathcal{X}\mathcal{Y}}$ by enforcing the prediction of target domain $\mathcal{Y}$ of $f_{\mathcal{X}\mathcal{Y}}$ and $f_{\mathcal{Y}_s\mathcal{Y}}\circ f_{\mathcal{X}\mathcal{Y}_s}$, where auxiliary domain $\mathcal{Y}_s$ is decomposed from the target domain $\mathcal{Y}$,  to be consistent.
%%%%%% 다른점 강조 더하기
% Different from cross-\textit{task} consistency, our cross-\textit{path} consistency learning does not require pre-trained models for each inference paths to impose consistency between them.
% Also, we augment the decoding path with intermediate output $y_s$ before final output where task consistency learning extends to another domain $y_a$ after the target domain.
Also, while cross-\textit{task} consistency learning requires the mapping function $f_{\mathcal{Y}\mathcal{Y}_a}$ to be pretrained to avoid suboptimal training with the noisy estimator, cross-\textit{path} consistency learning does not demand any task-specific pre-trained networks since the auxiliary domain $\mathcal{Y}_s$ is part of the target domain $\mathcal{Y}$. 
% Also, as shown in Figure~\ref{fig:consistency variants}, cross-task consistency uses auxiliary task $\mathcal{Y}_a$ which is extended from the target output to train the main task function $f_{\mathcal{X}\mathcal{Y}}$, whereas cross-path consistency augments the inference path with intermediate output $\mathcal{Y}_s$ to impose consistency across all paths. 
Details for our framework is described in section~\ref{section3.2}.

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/3_Method/3_1_Revisit_HOI_Transformer.tex <==
\section{Method}
In this section, we \hwan{describe our novel end-to-end training strategy for transformers with \textbf{cross-path consistency} in Human-Object Interaction Detection.}  
% In this section, we introduce our novel training strategy in detail. 
%We propose  for transformers with multi-path consistency in Human-Object Interaction Detection.
The training strategy includes 1) augmenting the decoding path and 2) consistency regularization between predictions of multiple paths. % path 에 대한 설명?
\hwan{In Section~\ref{section3.1}, we explain two general types of transformer in Human-Object Interaction detection.
Then, we describe how our two training strategies, decoding-path augmentation and cross-path consistency learning, in Section~\ref{section3.2} and Section~\ref{section3.3}.}
%Our training schema augment the decoding path to generate multiple paths to train a model.
%For HOI detection, we augmented a path and generated 3 extra paths to train a model. 
%And without any extra decoders for each path, model is trained with only one set of encoder 
%The purpose of our work is augmenting a decoding path to multiple paths 
\subsection{Revisit Transformer in HOI detection}
\label{section3.1}
% hoi transformer는 크게 두가지로 나눌 수 있다.  2decoder with instance matching , 1decoder 
%This section explains single decoder and two decoder HOI transformer models in detail to show how our training strategy can be applied to both transformer-based HOI detection models.%추가함 
%Extension upon DETR, existing HOI transformers are composed of backbone CNN followed by encoder-decoder architecture of transformer.

% \hwan{HOI transformers are commonly extended upon DETR~\cite{carion2020end}, which are composed of backbone CNN followed by encoder-decoder architecture of transformer~\cite{Vaswani17transformer}.}
% The backbone CNN first extracts \textit{locally aggregated} feature  from input image $x \in \mathbb R^{H \times W \times 3}$. 
% Then, \hwan{the extracted features $X\in \R^{H'\times W'\times D}$} are passed into an encoder of which self-attention to \textit{globally} aggregate features.
% %At the decoding stage, the encoder feature map $F_{\text{enc}}\in\R^{D\times H'\times W'}$ and learnable position encoding $\text{p}\in \R^{N_q\times D_\text{p}}$ are the input of a decoder.
% \hwan{%At the decoding stage, the decoder takes encoded features $X \in \R^{D\times H'\times W'}$ and learnable positional embedding $p \in  \R^{N_q\times D_\text{p}}$ to predict the HOI triples. 
% %Here, $N_q$ number of queries are updated with self-attention and co-attention to highliht a specific information of the encoded features.

% In the decoding stage, the majority of the HOI transformers can be divided into two types; predicting HOI triplets at once~\cite{tamura2021qpic,zou2021end} or separately~\cite{kim2021hotr,chen2021reformulating}. 
% We will explain about common characteristics and differences between the single-decoder models and the two-decoder models.
% }

\hkc{
HOI transformers are commonly extended upon DETR~\cite{carion2020end}, which is composed of a CNN backbone followed by the encoder-decoder architecture of Transformer~\cite{Vaswani17transformer}. The CNN backbone first extracts \textit{locally} aggregated feature from input image $x \in \mathbb R^{H \times W \times 3}$. 
Then, the extracted feature map $X\in \R^{H'\times W'\times D}$ are passed into the encoder to \textit{globally} aggregate features via the self-attention mechanism. 

% Finally, the densely encoded features are cross-attended with object queries in the decoder layers.

% In the decoding stage, the majority of the HOI transformers can be distinguished by how the HOI triplets are predicted; predicting HOI triplets at once~\cite{tamura2021qpic,zou2021end} or seperately~\cite{kim2021hotr,chen2021reformulating}. 
% The commonalities and differences of the single-decoder and two-decoder models will be summarized shortly.
}
\jhp{In a decoding stage, learnable query embeddings $p\in \R^{N\times D}$ are fed into 6-layer decoder and updated into $e\in\R^{N\times D}$ by interacting with encoded feature map $X$ through cross-attention. Basically at the end of each layer, feed-forward networks for each HOI triplet element is attached to localize human and object regression, and predict interaction classes. 

At the training phase, Hungarian algorithm is used to match between ground truth labels and predictions from the decoder, and calculate the loss between them. 
The predictions unmatched with ground truth labels are considered as no object and interactions.  

In the localizing part, simple extention from DETR~\cite{tamura2021qpic,zou2021end} is to directly regress the box coordinates of humans and objects. This brings out the problem that human or object can be redundantly predicted with multiple query embeddings since the ground truth set is composed of HOI triplets. Other variants~\cite{kim2021hotr,chen2021reformulating} overcome this issue to construct extra branch for instance detection and use matching scheme for binding the relevant instances from instance decoder outputs in interaction decoder outputs.

}

%Number($N_q$) of queries which are learnable position encoding are updated with self-attention layers and co-attention layers to highlight a certain area of the encoder feature map $F_{enc}$.  
%기존: At the decoding stage, decoder uses learnable position embeddings $\text{p}\in \R^{N_q\times D_\text{p}}$ which are specialized to certain areas in encoded feature map $F_{enc}\in\R^{D\times H'\times W'}$ to update query by using self-attention with themselves and co-attention with feature map $F_{enc}$. 
%The variants of HOI transformer can be divided into two types whether object detection and action classification is done seperately~\cite{kim2021hotr,chen2021reformulating} or not~\cite{tamura2021qpic,zou2021end}. 
%We will briefly explain about each types of HOI transformer architecture below.

\paragraph{Single Decoder HOI Transformer.}
\hwan{The single-decoder HOI transformers~\cite{tamura2021qpic,zou2021end} directly infer HOI triplets in the decoding stage.
They extend DETR with an additional readout function for action classification in the decoder head.  
The decoding stage of single decoder models can be written as 
\begin{equation}
    \label{eq:single_dec}
    \begin{split}
        e &= {\text{Dec}}(p,\ X), 
    \end{split}
\end{equation}
where $e$ denotes the output embeddings, and $p$ denotes the learnable position encoding for the query input.
Then, the output embeddings are passed into feed-forward networks (FFN) for bounding box regression and action classification, as shown below.
\begin{equation}
    \label{eq:single_ffn}
    \begin{split}
        \hat{b}_h &= \text{FFN}_{h}\left(e\right), \\
        \hat{b}_o &= \text{FFN}_{o}\left(e\right), \\
        % \text{FFN}_\text{o}\left(e\right)  \\
        %\hat{c}_o &= \text{FFN}_\text{cls}\left(e\right) \\ 
        \hat{c}_{act} &= \text{FFN}_{act}\left(e\right),
    \end{split}
\end{equation}
where $\hat{b}_h,\hat{b}_o$ denotes predicted bounding boxes for the detected human or object, and $\hat{c}_{act}$ denotes the corresponding action logit.
The overall loss consists of binary cross entropy for multi-label action classification, softmax cross entropy for object classification, and $L_1$ and GIoU loss for regression.
}%Dimension 없애도 될듯? 동의합니다 보감합니다
% Only difference between single decoder HOI transformer and DETR is that readout function for action classification is added on decoder head. 
% Formulation for single decoder architecture can be written as:
% \begin{equation}
%     F_{\text{enc}} = f_{\text{enc}}(F_{\text{cnn}})
% \end{equation}
% \begin{equation}
%     e=f_{\text{dec}}(p, F_{\text{enc}})
% \end{equation}
%Here, $F_{\text{cnn}}\in\R^{D_{\text{cnn}}\times H' \times W'}$, $F_{\text{enc}}\in\R^{D \times H' \times W'}$, $e\in\R^{N_q\times D}$ denotes CNN backbone feature, encoder feature map and output query embeddings respectively and $\posE$ denotes learnable position encoding for input query and $f_{\text{enc}},f_{\text{dec}}$ for encoder, decoder respectively.
% Then, the output query embeddings $e$ are put into feed-forward networks $\text{FFN}_\text{h-box}:\R^{D}\rightarrow \R^4$,  $\text{FFN}_\text{o-box}:\R^{D}\rightarrow\R^4$, $\text{FFN}_\text{o-cls}:\R^{D}\rightarrow\R^{C_o}$ and $\text{FFN}_\text{a}:\R^{D}\rightarrow\R^{C_a}$ to get bounding box
% \begin{equation}
%     \hat{b}_h=\text{FFN}_\text{hum box}\left(e\right) 
% \end{equation}
% \begin{equation}
%      \hat{c}_o, \hat{b}_o=\text{FFN}_\text{obj cls}\left(e\right) , \text{FFN}_\text{obj box}\left(e\right) 
% \end{equation}
% \begin{equation}
%     \hat{c}_i=\text{FFN}_\text{act}\left(e\right)
% \end{equation}
% $$\mathcal{L}=\lambda_a\cdot\mathcal{L}_a+\lambda_{\text{obj}}\cdot\mathcal{L}_{\text{obj}}+\lambda_{\text{bbox}}\cdot\mathcal{L}_{\text{bbox}}+\lambda_{\text{GIoU}}\cdot\mathcal{L}_{\text{GIoU}}$$

\paragraph{Two Decoder HOI Transformer.} 
%%%% 포괄하는 formulation FFN 부분을 
\hwan{
Despite the simple extension of single decoder HOI transformers, its architecture poses a problem that same human or objects can be redundantly inferred from different queries.
Therefore, two-decoder HOI transformers~\cite{kim2021hotr,chen2021reformulating} include two different parallel decoders: \jhp{ one for instance detection and the other for interaction detection.}
% Each decoder predicts instance and interaction separately.
\jhp{The instance decoder, which is only responsible for object detection, is frozen during training so that the quality of object detection does not affect HOI detection.
The interaction decoder infers interactions and creates semantic information for human and object, so that each interaction is matched to the relevant human and object derived from the instance decoder.}
The output embeddings can be obtained by
\begin{equation}
    \label{eq:two_dec}
    \begin{split}
        % F_{\text{enc}} &= f_{\text{enc}}(F_{\text{cnn}}) \\
        % e_{\text{ins}} &= f_{\text{dec}}(p, F_{\text{enc}}) \\
        % e_{\text{int}} &= f_{\text{dec}}\left(\posE,F_{\text{enc}}\right).
        % \\ 
        % \text{alternative, } \\
        e_{\text{ins}} &= {\text{Dec}_\text{ins}}(p,\ X), \\
        e_{\text{int}} &= {\text{Dec}_\text{int}}(p,\ X),
    \end{split}
\end{equation}
where $e_{\text{ins}}$, $e_{\text{int}}$ denotes output embeddings of instance decoder and interaction decoder respectively. 
\jhp{For the final predictions of HOI triplets, similarity matching (dot-product for HOTR~\cite{kim2021hotr} and $L_1$ distance for AS-NET ~\cite{chen2021reformulating}) is used between projected interaction embeddings and instance embeddings to predict \texttt{human} and \texttt{object}, and multi-label classification is done for \texttt{interaction}.}
% Similar to the single-decoder models, output query embeddings passed into the FFNs to predict the final outputs :
\jhp{
Final predictions can be written as
\begin{equation}
    \label{eq:two_ffn}
    \begin{split}
        \hat{b}_h &= \text{sim}\big(\text{FFN}_{h}\left(e_{\text{ins}}\right),\text{FFN}\left(e_{\text{int}}\right)\big), \\ \hat{b}_o &= \text{sim}\big(\text{FFN}_{o}\left(e_{\text{ins}}\right),\text{FFN}\left(e_{\text{int}}\right)\big),  \\
        %\hat{c}_o &= \text{FFN}_\text{cls}\left(e_{\text{ins}}\right) \\ 
        \hat{c}_{act} &= \text{FFN}_{act}\left(e_{\text{int}}\right)
    \end{split}
\end{equation} %note 용례 볼 것 \
$\text{FFN}_h$ and $\text{FFN}_o$ are the projection networks that keep the dimensionality of the output queries consistent.

Since two decoder architectures freeze parameters related to instance detection, no regression loss is used. HOTR and AS-NET use cross-entropy and $L_1$ distance for instance prediction ($\hat{b}_h,\hat{b}_o$)  respectively, and for multi-label action classification, binary cross entropy is used.}

% Note: Since each output embedding is independent, it needs to combine the most related queries between interaction decoder and instance decoder.
% Therefore, the two-decoder add a matching loss $\mathcal L_{\text{match}}$ which is the distance between $e_{\text{ins}}$ and $e_{\text{int}}$ to the total losses.


%Also,  is added on the losses of the single-decoder models to preserve the advantage of DETR; eliminating the post-processing.
%Here, the distance function can be either cosine similarity or $L_p$ norm.
% In order to preserve the advantage of DETR; eliminating the post-processing, overall losses for two-decoder models only added matching loss $\mathcal L_{\text{match}}$ on the top of the loss functions of the single-decoder models.
}

% Path-wise Loss is a supervision loss that is applied to each path. 
% For our model to learn with multiple paths, decoders $f_{i,j}$ from different paths and stages share their parameters. 
% In other words, model parameters are trained to optimize loss of all possible decoding paths. 
% % This allows the size of the model to remain the same as the baseline model whether it is single decoder model or two decoder model. 
% Each path is trained with supervision losses of bounding box $\mathcal{L}_b$ , object class $\mathcal{L}_c$ and action class $\mathcal{L}_a$.
% Bounding box regression loss $\mathcal{L}_b$ is calculated with $L_1$ loss and $GIoU$ to regress the bounding box of human and object. 
% For $\mathcal{L}_c$ and $\mathcal{L}_a$ Cross Entropy loss and Binary Cross Entropy loss are used for object classification and multi-label action classification. 

% The reason why the instance and interaction decoder are presented separately is that in the case of a single decoder, redundant human or object box may appear in multiple output queries when directly infer box coordinates.
%Two-decoder models~\cite{kim2021hotr,chen2021reformulating} seperately infer instance and interaction and bind the two outputs. 
% \begin{equation}
%     F_{enc} = f_{enc}(F_{cnn})
% \end{equation}
% \begin{equation}
%     e_{ins}=f_{dec}\left(\posE,F_{enc}\right)  
% \end{equation}
% \begin{equation}
%     e_{int}=f_{dec}\left(\posE,F_{enc}\right)  
% \end{equation}
%To bind the two independent outputs, distance are calculated between output embeddings from instance decoder and output embeddings from interaction decoder to match with lowest distance.
% Therefore, ~\cite{kim2021hotr,chen2021reformulating} uses matching strategy by calculating the distance bewteen output embeddings from instance decoder $v^{instance}\in \R^{M_q\times D}$ and output embeddings of human $v^{interact}_\text{h}\in \R^{N_q\times D}$ and object $v^{interact}_\text{o}\in \R^{N_q\times D}$ from interaction decoder.
% $M_q$, $N_q$ are number of queries in instance decoder and interaction decoder respectively.
% All those matching embeddings are projected from output queries by using feedforward network $\text{FFN}:\R^D\rightarrow\R^D$. 
%HOTR uses cosine similarity and AS-NET uses $L_1$ distance to select the most related human and object in interaction queries from instance detection results. 
%The final output predictions can be derived as follows: 
%Output embedding $e_{ins}$, $e_{int}$ are then put into feed-forward networks to retrieve \texttt{<human, verb,  object>} triplets:
% \begin{equation}
%     \hat{b}_h=\text{FFN}_\text{hum box}\left(e_{ins})\right) 
% \end{equation}
% \begin{equation}
%      \hat{c}_o, \hat{b}_o=\text{FFN}_\text{obj cls}\left(e_{ins}\right) , \text{FFN}_\text{obj box}\left(e_{ins}\right) 
% \end{equation}
% \begin{equation}
%     \hat{c}_i=\text{FFN}_\text{act}\left(e_{int}\right)
% \end{equation}
% Like single decoder architecture, $\text{FFN}_\text{act}:\R^D\rightarrow\R^{C_a}$ is used for action classification.
% The loss function of two decoder models consist of instance-interaction matching loss on top of single decoder loss function. 
% For the instance-interaction matching loss, HOTR and AS-NET uses NCE(?) and pull-push scheme respectively, to maximize agreement between the related instance embeddings and projected interaction embeddings of human and object.
%  In the case of loss fucntion, binary cross entropy is used for multi-label action classification like single decoder method and instance-interaction matching loss for prediction of human and object. For the matching loss function, HOTR and AS-NET uses NCE(?) and pull-push scheme respectively, to bring the related instance embeddings and projected interaction embeddings of human and object close together.      
% $$F_{enc}=\mathbf{Enc}\left( I \right)$$
% $$e^{interact}=\mathbf{Dec}_{interact}\left(\{\text{p}^{interact}\},F_\text{enc}\right)$$
% $$e^{instance}=\mathbf{Dec}_{instance}\left(\{\text{p}^{instance}\},F_\text{enc}\right)$$
% \begin{itemize}
%     \item \textbf{Output}\\
% $$\text{H}=\underset{j}{\operatorname{argmax}}\left(\text{sim}\left(\text{FFN}_{\text{sub}}\left(e^{interact}\right),e^{instance}_j\right)\right)$$ 
% $$\text{O}=\underset{j}{\operatorname{argmax}}\left(\text{sim}\left(\text{FFN}_{\text{obj}}\left(e^{interact}\right),e^{instance}_j\right)\right)$$ 
% $$\text{I}=\text{FFN}_\text{act}\left(e^{interact})\right)$$
%     \item \textbf{Loss}
%     $$\mathcal{L}=\lambda_a\cdot\mathcal{L}_a+\lambda_{\text{h}}\cdot\mathcal{L}_{\text{h}}+\lambda_{\text{o}}\cdot\mathcal{L}_{\text{o}}$$
% \end{itemize}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/3_Method/3_1_Revisit_HOI_trans_ver2.0.tex <==
\section{Method}
In this section, we present our novel end-to-end training strategy for Transformers with \textbf{cross-path consistency} in Human-Object Interaction Detection.
The training strategy includes 1) augmenting the decoding path and 2) consistency regularization between predictions of multiple decoding paths. 
Before discussing our training strategy, we briefly summarize transformers in Human-Object Interaction detection.

\subsection{Transformer in HOI detection}
\label{section3.1}
HOI transformers are commonly extended upon DETR~\cite{carion2020end}, which is composed of a CNN backbone followed by the encoder-decoder architecture of Transformer~\cite{Vaswani17transformer}. 
% The CNN backbone first extracts \textit{locally} aggregated features from input image $x \in \mathbb R^{H \times W \times 3}$. 
% Then, the extracted feature map $X\in \R^{H'\times W'\times D}$ is passed into the encoder to \textit{globally} aggregate features via the self-attention mechanism.
\jhprev{The CNN backbone first extracts a \textit{locally} aggregated feature map $f\in\R^{H'\times W' \times D}$ from input image $x \in \mathbb R^{H \times W \times 3}$.
Then, the feature map $f$ is passed into the encoder to \textit{globally} aggregate features via the self-attention mechanism, resulting in the encoded feature map $X\in\R^{H'\times W' \times D}.$
}
At a decoding stage, a decoder takes learnable query embeddings $\jhprev{q}\in \R^{N\times D}$ and outputs $e\in\R^{N\times D}$ by interacting with encoded feature map $X$ through cross-attention. 
The outputs are converted to final HOI predictions (\ie, human, object, interaction) by read-out functions, which are generally feed-forward networks. 

Training Transformers for detection entails matching between predictions and ground truth labels since Transformers provide detections as set predictions. 
To compute losses, the Hungarian algorithm~\cite{kuhn1955hungarian} is used to associate detections with ground truth labels.
The predictions unmatched with ground truth labels are considered as no object or no interactions.  
In general, HOI transformers can be categorized into two groups based on human/object localization schemes. 
\cite{tamura2021qpic,zou2021end} directly predict the box coordinates of human and object from an HOI prediction.
But this causes problems that human or object can be redundantly predicted by multiple query embeddings and the localizations of the same object often differ across HOI triplet predictions.
To address these problems, ~\cite{kim2021hotr,chen2021reformulating} propose parallel architectures to perform interaction detection separately from object detection.


% In the localizing part, simple extension from DETR~\cite{tamura2021qpic,zou2021end} is to directly regress the box coordinates of human and object. 
% This brings out the problem that human or object can be redundantly predicted with multiple query embeddings since the ground truth set is composed of HOI triplets.
% Other variants~\cite{kim2021hotr,chen2021reformulating} overcome this issue by constructing extra branch for instance detection and use matching scheme for binding the relevant instances from instance decoder in interaction decoder.



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/3_Method/3_2_Multi-Path_Inference.tex <==
\subsection{Decoding-Path Augmentation}
\label{section3.2}      
\input{Figure_caption/fig1_extension}
\input{Figure_caption/fig2}

We observe that HOI detection can be achieved by various sequences of predictions.
For instance, CNN-based HOI detection models~\cite{gkioxari2018detecting, chao2018learning, Gao2020DRG, gupta2019no} first detect instances (human and object) and then predict interactions between the instances, 
\ie, $x \rightarrow \text{HO} \rightarrow \text{I}$, where $x$ is an input image and H, O, I are predictions for human, object, interaction, respectively. 
On the other hand, the HOI Transformers by \cite{kim2021hotr,tamura2021qpic, chen2021reformulating, zou2021end} directly predict HOI triplets, \ie, $x \rightarrow \text{HOI}$.
Inspired by Cross-Task Consistency \cite{zhang2018deep} and this observation, 
we propose \textbf{decoding-path augmentation} to generate various decoding paths (or prediction paths) and impose consistency regularization.
Decoding-path augmentation for Transformers in HOI detection can be easily achieved by partially decoded HOI predictions.
Furthermore, sharing decoders across paths is beneficial in terms of knowledge sharing.

In our experiments, we consider four decoding paths as follows:
\begin{equation}
\begin{split}
    \label{eq:all_path}
    &\;\paths_1 = x \rightarrow \text{HOI} \\ 
    &\begin{rcases*}
    \paths_2 =x \rightarrow \text{HO} \rightarrow \text{I} \\ 
    \paths_3 = x\rightarrow \text{HI} \ \rightarrow \text{O} \\ 
    \paths_4 =x \rightarrow \text{OI} \ \rightarrow \text{H}
    \end{rcases*}
    Augmented.
\end{split}
\end{equation}

% \begin{equation}
%     \label{eq:all_path}
%     \paths_k =
%     \begin{cases}
%     Q_\phi \rightarrow Q_\text{HOI}, &k=1 \\ 
%     Q_\phi \rightarrow Q_\text{HO}  \rightarrow Q_\text{I}, &k=2 \\ 
%     Q_\phi \rightarrow Q_\text{HI}\ \rightarrow Q_\text{O}, &k=3 \\ 
%     Q_\phi \rightarrow Q_\text{OI}\ \rightarrow Q_\text{H}, &k=4
%     \end{cases}
% \end{equation}
% For brevity, we express the decoding stage in HOI transformers as $Q_a\rightarrow Q_b$.
% With the notations, the original decoding stage of the HOI transformers can be written as $Q_{\phi}\rightarrow Q_\text{HOI}$. $Q_\phi$ denotes a zero vector.

Each decoding stage of path $\paths_k$ can be written as:  
\begin{equation}
    \label{eq:path_decoding}
    \begin{split}
        e_{{k,1}} &= f(e_{k,0}+ q_{k,1}, \ X), \\
        e_{{k,2}} &= f(e_{k,1} + q_{k,2}, \ X),
    \end{split}
\end{equation}
where ${q}_{k,j}, \ e_{k,j}$ denote learnable query and output embeddings on $k^{\text{th}}$ path at $j^{\text{th}}$ decoding stage. The decoder $f$ is shared across all paths and stages.
The $e_{k,0}$ above is dummy output embeddings set to zeros since there is no 0-th stage, see Figure \ref{fig:pipeline}.
%Outputs of the last layer of $f_{k,1}$ serve as input queries for $f_{k,2}$.  
Each decoding stage and path use a separate readout function $\text{FFN}$ to translate the output embeddings into HOI instance predictions. 
For example, on $\paths_2: x \rightarrow \text{HO} \rightarrow \text{I}$, at stage 1
$e_{2,1}$ is read out by $\text{FFN}^{\paths_2}_{h}$ and $\text{FFN}_{o}^{\paths_2}$ to predict bounding boxes of human and object respectively.
 Prediction for HOI element \jhprev{$m \in \{h,o,act \}$} in each $k^{th}$ path at $j^{th}$ decoding stage can be written as $\hat{y}_{k}^m=\text{FFN}^{\paths_k}_m\left(e_{k,j}\right)$. 











==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/3_Method/3_3_Consistency_Learning.tex <==
\subsection{Cross-Path Consistency Learning}%%%%% figure 필요 설명위해서 
\label{section3.3}
\hjk{We now present our Cross-Path Consistency Learning framework (CPC) that imposes consistency regularization between predictions from different decoding paths as shown in Figure~\ref{fig:consistency for HOI}.
Learning with CPC leads better generalization without any additional data or labels. 

\paragraph{Cross-Path Consistency.}
We explain our consistency learning scheme with an exemplary case of main path $\paths_1$ and augmented path $\paths_2$ given as
\begin{equation}
\label{eq:path}
    \begin{split}
        &\paths_1 : x \rightarrow \text{HOI} \\ 
        &\paths_2 : x \rightarrow \text{HO} \rightarrow \text{I}. 
    \end{split}
\end{equation} 
Here, the main path $\paths_1$ is the HOI transformers' original inference path.
In path $\paths_2$, human and object detection logits $\hat{y}^h_2$ and $\hat{y}^o_2$ are obtained reading out $e_{2,1}$, which is the output embeddings on path 2 at stage 1. 
Then, the interaction logit $\hat{y}^{act}_2$ is obtained after another subsequent decoder pass defined as $f_{2,2}$.
The corresponding inference scheme of $\paths_2$ can be written in more formal terms:
\begin{equation}
\begin{split}
\label{eq:out2}
    \hat{y}_2^{h}&=\text{FFN}_h^{\paths_2}(f_{2,1}(X)) \\
    \hat{y}_2^{o}&=\text{FFN}_o^{\paths_2}(f_{2,1}(X)) \\
    \hat{y}_2^{act}&=\text{FFN}_{act}^{\paths_2}(f_{2,2}\circ f_{2,1}(X)) \\
\end{split}
\end{equation}
In ~\eqref{eq:out2}, input arrays for $f$ other than feature map $X$ were omitted for simplicity.

With the predictions, we impose regularization to make the outputs from path $\paths_1$ and path $\paths_2$ consistent. 
Note that HOI detections from $\paths_2$ consist of both final and intermediate decoder outputs.
To this end, we define the loss function $\mathcal{L}_{\paths_{1}\paths_2}$ by aggregating losses from multiple augmented paths to enforce consistency. 
The loss function is given as:
\begin{equation}
\begin{split}
     \mathcal{L}_{\paths_{1}\paths_2}=\lambda_h\cdot\mathcal{L}_{h}\big(\hat{y}_1^{h},\hat{y}_2^{h}\big)  +\lambda_o\cdot
     \mathcal{L}_{o}\big(\hat{y}_1^{o},\hat{y}_2^{o}\big) \\ +\lambda_{act}\cdot\mathcal{L}_{act}\big(\hat{y}_1^{act},\hat{y}_2^{act}\big),
\end{split}
\end{equation}
where $\hat{y}^h_1$, $\hat{y}^o_1$ and $\hat{y}^{act}_1$ are the output from the main path $\paths_1$ and $\lambda$ are the loss weights. 
In our experiments, softmax-type outputs use Jensen-Shannon divergence (JSD) for consistency loss to give loss to each path symmetrically, while outputs followed by sigmoid, \eg, box regression, multi-label action classes, take the Mean-Squared Error loss. 
More details on type-specific loss functions are in the supplement.

In the case of other path pairs, loss is computed in the same manner. The final loss should thus incorporate all possible pairs. Then, the cross-path consistency (CPC) loss can be written as:
\begin{equation}
\label{eq:cpcloss}
    \mathcal{L}_\textbf{CPC}=\frac{1}{S}\sum_{(k,k')\in
\mathcal{K}}\mathcal{L}_{\paths_k\paths_{k'}}
\end{equation}
where $\mathcal{K}$ denotes the set of all possible path pairs, and $S$ refers to the size of set $\mathcal{K}$, \ie the number of path combinations.}


\paragraph{Cross Matching.}
% Cross-Path Consistency Learning enforces outputs from different paths to be consistent.
% \textcolor{red}{Since HOI transformers reformulate HOI detection as direct set prediction, we cannot specify the prediction of HOI triplet for each query. 
% Thus, our cross-path consistency learning scheme cannot be employed without specification for the predicted set. 
% Therefore, we present \textbf{cross matching}, a technique to bind outputs from different paths.
% Cross matching gives an inductive bias that makes queries with the same HOI elements consistent.
% To this end, cross matching aggregates outputs with the same supervision.} % during ground truth matching.
\hjk{
Cross-path consistency learning encourages outputs from different paths to be consistent.
However, since the outputs from a path are given as a set, we first need to 
resolve correspondence to specify the pairs of predictions to enforce consistency.
We present \textbf{cross matching}, a simple method that tags each instance with its corresponding ground truth label. 
The instances tagged with the same label are paired to compute consistency loss.
On the other hand, if an instance is not matched with any of the paths' output, 
we simply exclude the instance from consistency learning treating it as \textit{no object} or \textit{no interaction}.
Our cross-path consistency loss is introduced below.
}

%%%%%%%%%%%%%%%%%%%%%
% \textcolor{cyan}{
% Cross-path consistency learning encourages outputs from different paths to be consistent.
% However, it is not straightforward to match instances across paths because the output of each path is a set. 
% Thus, we present \textbf{cross matching}, a simple method that tags each instance with its corresponding ground truth label. 
% The instances tagged with the same label are grouped to compute consistency loss.
% For the instances that are not matched with any of the paths' output, we relabel them \textit{no object} or \textit{no interaction} and exclude those instances from our consistency loss.
% Computation of our cross-path consistency loss is explained in detail with mathematical terms below.
% }
%%%%%%%%%%%%%%%%%%%%%


%Inverse does not exist unless it is one-to-one matching...


Let $\sigma_k(i)$ denote the index of the ground truth label that matches the $i^{th}$ query in the $k^{th}$ path. %, $\phi$: idx $\rightarrow$ idx is a matching function. 
We define $\sigma_{k}^{-1}\left(n\right)$ as the query index of path $\paths_k$ which is matched with the ground truth index $n$.
To avoid clutter, we use  $\tilde\sigma_{k,n}$ as a shorthand notation for $\sigma_{k}^{-1}\left(n\right)$.
The outputs from different paths with the same ground-truth label should be consistent. 
For example, $\hat y^m_{k, {\tilde{\sigma}_{k,n}}}$ and $\hat y^m_{k, {\tilde{\sigma}_{k^\prime,n}}}$ which are predictions for $m$ from $\paths_k$ and $\paths_{k^\prime}$ with the same ground-truth index $n$ should be consistent.   
% The outputs in $\{\hat{y}_{k,\tilde\sigma_{k,n}}\}_{k=1}^K$ should be consistent with one another, where $\hat{y}_{k,j}$ refers to the prediction of $j^{th}$ query in $k^{th}$ path.
% \textcolor{red}{As aforementioned, the outputs unmatched with ground truth labels are considered as no object or no interaction. We did not impose the cross-path consistency loss on the unmatched outputs.}

Cross-path consistency loss between output predictions from $\paths_k$ and $\paths_{k'}$ with the same ground-truth with index $n$ is defined as follows:
\begin{equation}
\begin{split}
    \mathcal{L}_{\paths_{k}\paths_{k'}}^n
    =  &\hspace{2mm} \lambda_h\cdot\mathcal{L}_{h}\big(\hat{y}^{h}_{k,\tilde\sigma_{k,n}},\hat{y}^{h}_{k',\tilde\sigma_{k',n}}\big) \\
    & + \lambda_o\cdot\mathcal{L}_{o}\big(\hat{y}^{o}_{k,\tilde\sigma_{k,n}},\hat{y}^{o}_{k',\tilde\sigma_{k',n}}\big) \\ 
    & + \lambda_{act}\cdot \mathcal{L}_{act}\big(\hat{y}^{act}_{k,\tilde\sigma_{k,n}},\hat{y}^{act}_{k',\tilde\sigma_{k',n}}\big)  
\end{split}
\end{equation}

\paragraph{Final Loss}
The final cross-path consistency loss for all $\paths_k$ is derived as,
\begin{equation}
    \mathcal{L}_{\textbf{CPC}}=\frac{1}{{S}\cdot\mathcal{N}}\sum_{n=1}^\mathcal{N}\sum_{(k,k')\in \mathcal{K}}\mathcal{L}_{\paths_{k}\paths_{k'}}^n
\end{equation}
where $\mathcal{N}$ is the number of ground truth labels.
Then, the final form of our training loss $\mathcal{L}$ is defined by
\begin{equation}
    \mathcal{L}=\sum_k\mathcal{L}_{\mathbf{sup}}^k+w(t)\cdot\mathcal{L}_{\textbf{CPC}},
\end{equation}
where $\mathcal{L}_\mathbf{sup}^k$ is the supervision loss for each path $\paths_k$ and $w(t)$ is a ramp-up function~\cite{laine2016temporal,berthelot2019mixmatch,tarvainen2017mean} for stable training.
Our overall framework is illustrated in Figure ~\ref{fig1}.



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/3_Method/3_4_Overall_Arch.tex <==
% \subsection{Overall Architecure}
% Figure \ref{fig1}, illustrates the overall architecture of Cross-Path Consistency Learning. 
% From the same input image $x$ multiple decoding paths $\{P_1, ... P_k, P_{k'}\} $ are augmented with Decoding-Path Augmentation introduced in section ~\ref{section3.2}. 
% Each path is trained with same Transformer Decoder $f$ that shares parameters, but to distinguish each decoding path $i$ and training stage $j$ we denote Transformer Decoder with $f_{i,j}$.
% Transformer Decoder takes input $x$ with different learnable position encodings $p_{i,j}$ for decoding path $i$ and training stage $j$. 
% Then outputs from Transformer Decoder $e_{i,j}$ is put in to feed-forward network for action classification, instance classification and box regression. 
% Each output from feed-forward network is matched with ground truth label $y_n$ by bipartite matching using Hungarian algorithm .
% The outputs that are matched with ground truth label $y_n$ denoted as $\hat{y}_{\tilde\sigma_{k,n}}$ are trained with supervision losses described in section ~\ref{}. 
% Also, those outputs that are matched with the same ground truth $\{\hat{y}_{\tilde\sigma_{k,n}}, \hat{y}_{\tilde\sigma_{k',n}}, ... \}$ are trained with Cross-Path Consistency Loss described in section ~\ref{}. 


==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/4_Experiment/4_1_Dataset.tex <==
\section{Experiments}

In this section, we empirically evaluate the effectiveness of our cross-path consistency learning with HOI transformers. 
Our experiments are conducted on public HOI detection benchmark datasets: \textbf{V-COCO} and \textbf{HICO-DET}.
We first briefly introduce the datasets and provide implementation details.
Our extensive experiments demonstrate that our training strategy renders significant improvement on the baseline models without additional parameters or inference time. 

\subsection{Dataset}
\paragraph{V-COCO}~\cite{gupta2015visual} is a subset of the COCO dataset~\cite{lin2014mscoco} which contains 5,400 \texttt{trainval} images and 4,946 \texttt{test} images.
V-COCO is annotated with 29 common action classes.
For evaluation of the V-COCO dataset, we report the mAP metric over 25 interactions for two scenarios, 
% \textcolor{red}{excluding the interaction \textit{point} during the inference because only 31 instances appear in the test set.}
The first scenario includes a prediction of occluded objects and is evaluated with respect to {AP}${}^{}_{\text{role1}}$. 
On the other hand, the second scenario does not contain such cases, and performance is measured in {AP}${}^{}_{\text{role2}}$.   


\paragraph{HICO-DET}~\cite{chao2018learning} is a subset of the HICO dataset which has more than 150K annotated instances of human-object pairs in 47,051 images (37,536 for training and 9,515 for testing). 
It is annotated with 600 $\texttt{<interaction, object>}$ instances.
There are 80 unique object types, identical to the COCO object categories, and 117 unique interaction verbs.
For evaluation of the HICO-DET, we report the mAP over three different set categories: (1) all 600 HOI categories in HICO (Full), (2) 138 HOI categories with less than 10 training samples (Rare), and (3) 462 HOI categories with more than 10 training samples (Non-Rare).
% \subsubsection{Dense HICO-DET}
% HICO-DET datset~\cite{} which is a large-scale benchmark for HOI detection have contributed largely to HOI detection research.  
% Annotations of HOI detection datasets include instances in image and interaction pair of human and object instances with action class. 
% This complex annotations make difficult to annotate all possible interactions in the image.
% In HICO-DET dataset not all of the interactions in the image are annotated.
% To test our model more accurately, we densely annotated the test dataset of HICO-DET. 
% % Our training strategy allows the model to learn from sparsely annotated data and perform well on the densely annotated test dataset. 
% By training models with sparsely annotated dataset and testing on our densely annotated dataset, can develop model for detecting densely located interactions in real-world. 

% \textbf{Dense annotation}. 
% %표 넣기 .. 
% %그림 넣기.. 

% Our dataset was annotated by 10 annotators with 3 people to confirm the annotations.
% Class of the \texttt{<human,  verb, object>} triplet remained the same and distribution of the label remained similar to the previous HICO-DET test-set.
% In table ~\ref{}, shows the increase in hoi annotations from 0 to 0.
% We hope this dataset will help development of the HOI detection research that can be applicable to dense visual relation detection in real-world. 


%HOI detection 이 annotate 해야하는것
%annotate 모든 annotation 을 하기에는복잡해서 다하기 어렵고 불가능하다. 
% we constructed densly annotated hico-det dataset 
% 10명 annotator, 3명의 검수자
%그림 예시 기존 그리고 새로운것.. 
%비교 annotation 수 class 별 비교표 
%기존 annotation 클래스를 유지하며 annotation 함

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/4_Experiment/4_2_Implementation_detail.tex <==
\subsection{Implementation Details}
% 우리 실험은 
\paragraph{Training}
In our experiment, QPIC~\cite{tamura2021qpic} and HOTR~\cite{kim2021hotr} were used as the baseline for the HOI transformer respectively.
During training, we initialize the network with pretrained DETR~\cite{carion2020end} on MS-COCO with a Resnet-50 backbone.
For all decoding paths, parameters of the model are shared except for stage-wise queries and feedforward networks.

All our experiments using consistency regularization are trained for 90 epochs and the learning rate is decayed at the 60-th epoch by a factor of 0.1. 
As an exception, HOTR is trained up to 50 epochs and the learning rate is decayed at epoch 30 by a factor of 0.1  for HICO-DET.
Following the original training schemes in QPIC and HOTR, we freeze the encoder and backbone for HOTR, whereas unfreeze those for QPIC.
We use the AdamW~\cite{loshchilov2017decoupled} optimizer with a batch size of 16, and the initial learning rates for the transformer and backbone parameters are set to $10^{-4}$ and $10^{-5}$ respectively, and weight decay is set to $10^{-4}$. 
All experiments are trained on 8 V100 GPUs.

We re-implement the result of QPIC and HOTR on V-COCO~\cite{gupta2015visual}  since our reproduction results are quite different from the official ones in the paper.
For a fair comparison, all the loss coefficients overlapping between baselines and our training strategy are identical to the ones reported in the paper~\cite{kim2021hotr,tamura2021qpic}.
Details for hyperparameters relevant to our training strategy are reported in the supplementary material.
\paragraph{Inference} %
We mainly use $\paths_1$ ( $x\rightarrow \text{HOI}$ ) for inference to compare with the baseline models without increasing the number of parameters.
% For the compariaon with vanilla HOI transformers, we use $Q_X\rightarrow Q_\text{HOI}$ for inference, which is identical to the baselines, to have no additional computation cost. 
Also, we report the results of other inference paths in our ablation studies. 
% \textcolor{red}{All experiments are evaluated on 8 V100 GPUs.}
% \input{Table/HICO_new}

% \input{Table/Vcoco}



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/4_Experiment/4_3_Comparison_with_TR.tex <==
\subsection{Comparison with HOI transformer}
% \begin{table}[h]
    
        
    
%     \centering
%     \footnotesize
%     % \caption{Ablation.}
%     \label{tab:comp}
    
%     \begin{tabularx}{0.5\textwidth }{c | c c | c  c c }
%          \toprule
%          Method & \textit{AP}${}^{\#1}_{\text{role}}$ & 
%     \textit{AP}${}^{\#2}_{\text{role}}$ & F & R & NR\hspace{3pt} \\  
%          \midrule
         
%         QPIC & 58.8& 61.0 &29.07 &21.85& 31.23\hspace{3pt} \\
%         QPIC + ours & 63.11 & 65.44& 29.63&23.14 &31.57\hspace{3pt}  \\
         
%          \midrule
         
%          HOTR& 55.2 & 64.4 &25.10& 17.34&27.42\hspace{3pt}  \\
         
%          HOTR + ours& 61.60 &66.84 &26.16 &22.84 &27.15\hspace{3pt}\\
         
         
%          \bottomrule
%     \end{tabularx}
%     \caption{Comparison of our training strategy with vanilla HOI transformers on V-COCO and HICO-DET. * is our reproduction result with official code.}
%     \label{tab:cls}
    
% \end{table}
%As our training method is for transformer architecture, 
We evaluate the effectiveness of our method compared to the existing HOI transformers.
All experiments are reported with the main path $\paths_1$ that infers HOI triplets by a single decoding stage ($x\rightarrow\text{HOI}$) which is identical to the original HOI transformer.
As shown in Table~\ref{table:comp}, our CPC training strategy significantly outperforms on two baselines, HOTR~\cite{kim2021hotr} and QPIC~\cite{tamura2021qpic}.
% Such improvements may depict that the proposed learning strategy improves the generalization of the baseline architecture.  
In the V-COCO dataset, the experiment shows improvement in performance by a considerable margin of 0.9 mAP for QPIC in {AP}${}^{}_{\text{role1}}$, and 1.8 mAP for HOTR.
For {AP}${}^{}_{\text{role2}}$, QPIC and HOTR gain improvement by 0.9 mAP and 1.9 mAP respectively, similar to that of AP$_\text{role1}$.  

% In the HICO-DET dataset, QPIC outperforms all the evaluation categories and HOTR shows improvement in Full and Rare.
In the HICO-DET dataset, our CPC learning with HOTR and QPIC outperforms all the evaluation categories of HICO-DET, except negligible degradation in the Non-Rare category on HOTR.
Results on rare class on the HICO-DET are improved by a significant margin of 1.29 mAP and 5.5 mAP for QPIC and HOTR respectively.
In both models, we observe a more prominent performance improvement in the Rare category.
% It may support our training strategy is more flexible to learn for rarely seen triplets.
This supports that our training strategy performs well on rarely seen examples.
Our strategy improves the conventional HOI transformer models.
% Overall, experiment results imply that our training strategy can be applied to both one-decoder HOI transformer detector and two-decoder HOI transformer detector. 
\input{Table/main_short}
\input{Table/Vcoco}
\input{Table/HICO_new}
\input{Table/ablation_pathwise_noS2}


==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/4_Experiment/4_4_Comparison_with_SOTA.tex <==
\subsection{Comparison with State-of-the-Art Methods}
%We experimented our method on HICO-DET and V-COCO benchmarks to show the effectiveness of our training strategy
% Our training strategy achieves a new state-of-the-art performance on both V-COCO and HICO-DET bench marks. 
% Here, we compare previous HOI detection methods. 
In Table~\ref{tab:V-COCO} and Table~\ref{tab:HICO-DET}, we compare previous HOI detection methods with ours.
% performance on the V-COCO and HICO-DET test sets are compared. 
% All 
As demonstrated in the tables, our training strategy achieves the best performance among its peers.
Table~\ref{tab:V-COCO} shows the result on V-COCO dataset in both {AP}${}^{}_{\text{role1}}$ and {AP}${}^{}_{\text{role2}}$.
In the V-COCO dataset, our method achieves outstanding performance of 63.1 mAP in {AP}${}^{}_{\text{role1}}$ and 66.8 mAP in {AP}${}^{}_{\text{role2}}$. 
Also, the results on the HICO-DET dataset in Table~\ref{tab:HICO-DET} show that our CPC further improves the state-of-the-art models (\eg, HOTR, and QPIC) in the default setting achieving 26.16 mAP and 29.63 mAP, respectively.

% \input{Table/Vcoco}







==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/4_Experiment/4_5_1_Ablation_study.tex <==
\subsection{Ablation Study}
We further discuss the effectiveness of our framework through a series of ablation studies.
We first provide a path-wise analysis for our cross-path consistency learning method.
The effect of our training technique components was tested on each path to validate our method.
Subsequently, we analyze the impact of the number of augmented paths on the main task performance. 
We experimentally prove the validity of our method by demonstrating the correlation between the number of paths and performance.

\paragraph{Efficiency of CPC.}
% S1 + S2 version
% \input{Table/ablation_pathwise}
% \input{Table/ablation_pathnum}
% S1 only version
Table~\ref{table:abl} presents ablation experiment results for all inference paths, $\paths_1$, $\paths_2$, $\paths_3$, and $\paths_4$.
Path $\paths_1$ is the main path, which we aim to boost performance with the rest of the augmented paths.
% The first row of each method shows the results for each path when trained independently without parameter sharing. 
% The rest of our experiments are conducted with shared encoders.
We try ablating decoder sharing or cross-path consistency regularization one at a time to confirm each component's contribution to our training strategy.
Note that all of our experiments are conducted with the encoder block shared across paths.

When our CPC training strategies are applied, QPIC and HOTR achieve an mAP of 63.1, and 61.6 on main path $\paths_1$.
% Both HOTR and QPIC show the best performance on main path $\paths_1$ in the baseline.
% By sharing decoders without cross-path consistency, QPIC performs worse by 1.5 mAP , whereas HOTR outperforms by 0.8 mAP compared to the original setting of $\paths_1$. 
When the decoder parameters are not shared, performance degradation in path $\paths_1$ was observed for both baselines; a 0.7 mAP drop for QPIC, and 0.4  mAP drop for HOTR. 
On the other hand, when CPC regularization is left out while decoder parameters are shared, performance of QPIC and HOTR decreased by a large margin of 2.4 mAP and 1.0 mAP each. 
In terms of overall performance across all paths, the average mAP showed a similar trend for each experiment condition.
The overall results support that our learning strategy improves generalization of base architectures, and boosts performance by sharing knowledge throughout paths and stages.

% By applying CPC with unshared decoders for all stages, there was an average performance gain of 1.83 mAP on HOTR, whereas a slight decay in performance was observed in the case of QPIC compared to the original setting of average of all paths.
% However, when our CPC learning is applied with parameter sharing, both models achieve better performance throughout all path variants. 
% On average, our CPC learning strategy with shared decoders outperforms the independent-training strategy by 1.58 mAP for QPIC, and 2.28 mAP for HOTR compared to the original setting of average of all paths. 
% Compared to the unshared decoder setting, our method excels by a margin of 1.75 mAP for QPIC, and 0.45 mAP for HOTR.
% 여기는 숫자 deviation 둘다비교 
Interestingly, the standard deviation of all performances dramatically increases without both components.
With unshared decoders, deviation increases by 1.33 for QPIC and 0.35 for HOTR.
Also, when CPC regularization is removed, deviation increases by 1.01 for QPIC and 0.11 for HOTR. 
This implies that our training strategy with shared decoder and CPC leads to more stable training as well as consistent representations.

% without share deocder : 0.69 $\rightarrow$ 0.05 for QPIC and 0.37 $\rightarrow$ 0.02 for HOTR 
% without CPC: 0.69 $\rightarrow$ 0.05 for QPIC and 0.37 $\rightarrow$ 0.02 for HOTR .
% But for CPC learning with unshared decoder, the deviation of average performance in HOTR remains almost the same and increases for QPIC. 
% This implies that our learning strategy with shared decoder encourages learning of consistent representations. 


%11/14 17시 수정
% Table~\ref{table:abl} presents ablation results for other inference paths, $\paths_2$,$\paths_3$ and $\paths_4$ on the V-COCO dataset. 
% The top row for each method are the results for each path by training seperately.
% Both HOTR and QPIC basically show best performance in a main branch $\paths_1$. 
% By sharing parameters of all decoding paths without cross-path consistency, QPIC performs worse by 1.72 AP in \textit{AP}${}^{\#1}_{\text{role}}$ whereas HOTR gets better $\textit{AP}{}^{\#1}_{\text{role}}$ by margin of 1.45 AP. 
% When our training strategy is applied, both models achieve better performance across all the paths. 
% On average, our training strategy performs better than seperately trained paths by 1.63 AP for QPIC and 2.27 AP for HOTR in \textit{AP}${}^{\#1}_{\text{role}}$.
% Interestingly, the deviation between each path also decreased: 0.66 $\rightarrow$ 0.10 for QPIC and 0.48 $\rightarrow$ 0.05 for HOTR in \textit{AP}${}^{\#1}_{\text{role}}$. 
 %Those comparisons claim that our learning strategy makes all the different paths cosistent and improve generalization by a single estimator(or without increasing model complexity). 


==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/4_Experiment/4_5_2_Ablation_study.tex <==

\paragraph{Impact of Augmented Paths.}
% \input{Table/ablation_pathnum_noS2}
We explore how the number of augmented paths affects the performance of the main path $\paths_1$ in V-COCO benchmark.
Starting from $\paths_1$, the augmented paths are gradually added with respect to mAP of Scenario 1 from Table~\ref{table:abl_pathwise_sep}, where each path is independently trained with default settings with no training techniques applied.
We leverage the augmented path with better performance first, as performance of each model will serve as a lower bound for the ensemble of paths.
% Since it is reasonable to think that leveraging the path of good performance when trained seperately, we gradually add augmented path in the order of good performance.
Specifically, as shown in Table~\ref{table:abl_pathwise_sep}, both HOTR and QPIC showed better performance in the order of $\paths_1$, $\paths_2$, $\paths_3$, and $\paths_4$, when trained independently.

We compare the four cases where the augmented paths are gradually added in the corresponding order; \ie, $\paths_1$, $\paths_1+\paths_2$, $\paths_1+\paths_2+\paths_3$, and $\paths_1+\paths_2+\paths_3+\paths_4$.
As shown in Figure~\ref{fig:pathnum ablation}, performance is gradually improved as augmented paths are  added.
% In Table~\ref{table:abl_num}, as the augmented path adds up in consistency learning, performance of main path $\paths_1$ increases.
The ablation study evidences that regardless of each path performance, taking advantage of more paths bolsters the learning capability of our main task, and its performance builds up as the number of augmented paths increases.
% This ablation study strongly argue that whether the performance of the individual path is good or bad, using more path in our consisteny learning is better to have good performance.  
% {AP}${}^{}_{\text{role1}}$
\input{Table/ablation1_pathwise_seperate}
\vspace{-1.5mm}
\input{Figure_caption/pathnum_ablation}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/5_Conclusion/5_Conclusion.tex <==
\section{Conclusion}
% This paper present effective end-to-end training scheme for transformer in human object interaction by cross-path consistency learning.
% Cross-path consistency learning is a new consistency regularization method that augment the decoding paths and impose consistency regularization between them to supplement the all inference paths.
% Our training strategy is applicable to all transformer architectures that include decoding stages to make predictions and it does not effect the model complexity during the inference. 
% We validate the effectiveness of our approach by best result on two benchmark datset and verified the path consistency by our experiments. 
% In future works, we will apply our method to wider domain in computer vision.
 % end to end training schema for tranforemr 
 % Cross pat
 
We propose end-to-end Cross-Path Consistency learning for Human-Object Interaction detection. Through decoding-path augmentation, various decoder paths are generated which predict HOI triplets in permuted sequences. Then, consistency regularization is applied across paths to enforce the predictions to be consistent. Parameter sharing and cross-matching were introduced as well to enhance learning. 

Our method is conceptually simple, and can be applied to a wide range of transformer architectures. Also, it does not require additional model capacity nor inference time. The substantial improvements on V-COCO and HICO-DET support our method's efficacy in various HOI detection tasks. Through further empirical studies, its capabilities to improve generalization and to encourage consistent representations are approved. 
% We briefly discuss the limitations of our work below.

% supple로 이동 (camera ready)
% Apart from no additional computation at inference, the training complexity of our method scales linearly as the number of paths is augmented.
% In addition, our method mainly targets the HOI detection task; applications on simpler yet more general tasks as image classification or object detection were not covered in our work. Regarding our decoding-path augmentation method, further discussions on how our methods should be applied to tasks with non-separable output (\eg image classification) are required. This may be one interesting future direction of our work.   

% \hkc{We propose a novel end-to-end learning strategy called Cross-Path Consistency (CPC) learning for Transformer in Human-Object Interaction detection. 
% With a decoding-path augmentation, which augments the prediction of HOI to the different inference paths, we augments the HOI prediction and predict separate outputs.  
% Then, each output is enforced to be consistent with respect to the same ground-truth label.
% CPC learning trains the network only during the training without any additional parameter, and preserve the same inference time with significant improved accuaracy.  
%Through decoding-path augmentation, various decoding paths are generated which predict HOI triplets in permuted sequences. 
%Then, consistency regularization is applied across paths to enforce the predictions to be consistent. Key techniques as parameter sharing and cross matching were introduced as well to enhance learning. 
% Since our method is transforer-agnostic and can be applied 
% Our method is simple, and can be applied to a wide range of transformer architectures. Also, it does not require additional model capacity nor inference time. The substantial improvements on V-COCO and HICO-DET supports our method's efficacy in various HOI detection benchmarks, and its capability of improving generalization and encouraging consistent representations are approved through further empirical studies.
% However, our work bears limitation in its training efficiency, and in the range of task on which our method was experimented.
% 할거남앗어?
% \jhp{We describe some limitations in our learning strategy as below.
% \paragraph{Training efficiency}
% Our training scheme takes extra resourses compare to the baseline model we attached to, since 
% }


\input{5_Conclusion/Acknowledgments}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/5_Conclusion/Acknowledgments.tex <==
% \vspace{-1.5mm}
\paragraph{Acknowledgements}
This work was partly supported by Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (No.2021-0-02312, Efficient Meta-learning Based Training Method and Multipurpose Multi-modal Artificial Neural Networks for Drone AI), (IITP-2022-2020-0-01819, the ICT Creative Consilience program); ETRI grant (22ZS1200, Fundamental Technology Research for Human-Centric Autonomous Intelligent System); and KakaoBrain corporation.

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/5_Conclusion/CO.tex <==
\subsection{Conclusion and Limitations}
In this paper, we introduced Cross-Path Consistency Learning, novel end-to-end training strategy for general transformer architecture using consistency regularization in Human-Object Interaction detection. 
Our learning scheme leverages inference paths of difference sequence by augmenting the decoding path and imposes their predictions to be consistent, which leads to better generalization without increasing model capacity.
In the future work, we aim to apply our learning strategy for the general task, not limited to HOI, and more diverse transformer architecture.
We 


==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/5_Conclusion/HKC.tex <==
\section{Conclusion}
We proposed Cross-Path Consistency learning for Human-Object Interaction detection. Through decoding-path augmentation, various decoder paths are generated which predict HOI instances in permuted sequences. Then, consistency regularization is applied path-wise to impose consistency in the predicted HOI triplets, enforcing the predictions to be inference-path invariant. Key techniques as parameter sharing and cross matching were introduced as well to enhance learning. 

Our method is conceptually simple, and can be applied to a wide range of transformer architectures. Also, it does not require additional model capacity nor inference time. The state-of-the-art results on V-COCO and HICO-DET supports our method's efficacy in various HOI detection tasks, and its robustness is approved through further empirical studies.

However, our work's limitation lies in the task on which our method was experimented. HOI detection being an intricate vision task, it is yet relatively minor. That is, our method's feasibility in simpler and more general vision tasks was not thoroughly discussed in our work. Future work is called for.

% 1. CPC for HOI
% 2. Deocding-Path Augmentation
% 3. CPC and Cross Matching
% 4. sota performance V-COCO and HICO-DET
% 5. Limitations : narrow application 

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Figure_caption/fig1_extension.tex <==
\begin{figure}[tp]
\begin{subfigure}[t]{.49\linewidth}
\includegraphics[width=\textwidth]{Figure/aug_main.png}
\caption{}
\end{subfigure}
\begin{subfigure}[t]{.49\linewidth}
\includegraphics[width=\textwidth]{Figure/aug_aug.png}
\caption{}
\end{subfigure}
\caption{\textbf{Cross-path consistency for HOI detection}. (a) Main task path ${\color{red}\mathcal{P}_1}$ should be consistent with each augmented path. \eg path ${\color{blue}\mathcal{P}_2}$. (b) Augmented paths should be consistent with one another. \eg path ${\color{blue}\mathcal{P}_2}$ and ${\color{red}\mathcal{P}_3}$. }
\label{fig:consistency for HOI}
\end{figure}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Figure_caption/fig2.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figure/fig2_dot.png}
    % \vspace{-12pt}
    \caption{
    \label{fig:pipeline}
    {\textbf{The overall process of Cross-Path Consistency Learning}. The encoded image features are passed into the shared decoder with multiple inference paths $\{\paths_1, ..., \paths_{k-1}, \paths_k\}$. 
    Each path is augmented based on the decoding-path augmentation to generate various sequences of inference paths (see Section~\ref{section3.2}). 
    To avoid clutter, we visualize only the main path $\paths_1$ and an augmented path $\paths_k$. 
    The main path $\paths_1$ consists of a single decoding stage,
    % decoder $f_{1,1}$, 
    and the augmented path $\paths_k$ is a composition of decoding stages; all $f$ blocks share parameters.
    % two decoders $f_{k,1}$ and $f_{k,2}$; all $f_{k,j}$ share parameters. 
    Given queries $q$ a learnable position embeddings, each decoder extracts output embeddings denoted as $e_{1,1}$, $e_{k,1}$, and $e_{k,2}$. 
    Then, each of the output embeddings is fed into the readout function $\text{FFN}$ to predict each HOI element \ie \texttt{<human, object, interaction>}. 
    With Cross-Path Consistency Learning (Section ~\ref{section3.3}), all the outputs supervised with the same ground truth label are trained to be consistent regardless of their inference paths. 
    %바꿈 밑에 꺼랑 
    Cross-Matching is used to match the queries that are considered to be consistent by leveraging ground truth label. 
    % Here, queries that are matched with the same ground truth are considered to be trained to have the same semantic information, so that Cross-Matching scheme is used. 
    Along with the supervision loss $\mathcal{L}_\mathbf{sup}^k$ for all paths $\paths_k$, cross-path consistency loss $\mathcal{L}_\textbf{CPC}$ is added to our final loss.}}
% Multiple inference paths $\{P_1, ... P_{k'}, P_k\} $ are augmented with Decoding-Path Augmentation as introduced in section ~\ref{section3.2}. 
% % Each path is trained with the same Transformer Decoder $f$ that shares parameters, but to distinguish each decoding path $i$ and training stage $j$ we denote Transformer Decoder with $f_{i,j}$.
% % Transformer Decoder takes input $x$ with different learnable position encodings $p_{i,j}$ for decoding path $i$ and training stage $j$. 
% % Then outputs from Transformer Decoder $f_{i,j}(x,p_{i,j})=e_{i,j}$ are put in to feed-forward network for action classification, instance classification and box regression.
% \jhp{Each decoding stage $f_{k,j}$ extracts different semantic information that does not overlap with other decoding stage within the path. 
% At each $j^{th}$ decoding stage at $i^{th}$ path, transformer decoder takes input queries $Q_x$ with semantic queries $p_{i,j}$ and updated with encoder feature map $X$ through multi-head attention. 
% Those output queries $e_{i,j}$ are fed into feed-forward network(s) that fits the semantic information(s) in $e_{i,j}$. }
% Each output from feed-forward network is matched with ground truth label $y_n$ by bipartite matching using Hungarian algorithm .
% The outputs that are matched with ground truth label $y_n$ denoted as $\hat{y}_{\tilde\sigma_{k,n}}$ are trained with supervision losses. 
% Also, those outputs that are matched with the same ground truth $\{\hat{y}_{\tilde\sigma_{k,n}}, \hat{y}_{\tilde\sigma_{k',n}}, ... \}$ are trained with Cross-Path Consistency Loss described in section ~\ref{section3.3}. }

% 11/15 17시 수정
%     \caption{Overall architecture of Cross-Path Consistency Learning. 
% Multiple inference paths $\{P_1, ... P_k, P_{k'}\} $ are augmented with Decoding-Path Augmentation as introduced in section ~\ref{section3.2}. 
% % Each path is trained with the same Transformer Decoder $f$ that shares parameters, but to distinguish each decoding path $i$ and training stage $j$ we denote Transformer Decoder with $f_{i,j}$.
% % Transformer Decoder takes input $x$ with different learnable position encodings $p_{i,j}$ for decoding path $i$ and training stage $j$. 
% % Then outputs from Transformer Decoder $f_{i,j}(x,p_{i,j})=e_{i,j}$ are put in to feed-forward network for action classification, instance classification and box regression.
% \jhp{Each decoding stage $f_{k,j}$ extracts different semantic information that does not overlap with other decoding stage within the path. 
% At each $j^{th}$ decoding stage at $i^{th}$ path, transformer decoder takes input queries $Q_x$ with semantic queries $p_{i,j}$ and updated with encoder feature map $X$ through multi-head attention. 
% Those output queries $e_{i,j}$ are fed into feed-forward network(s) that fits the semantic information(s) in $e_{i,j}$. }
% Each output from feed-forward network is matched with ground truth label $y_n$ by bipartite matching using Hungarian algorithm .
% The outputs that are matched with ground truth label $y_n$ denoted as $\hat{y}_{\tilde\sigma_{k,n}}$ are trained with supervision losses. 
% Also, those outputs that are matched with the same ground truth $\{\hat{y}_{\tilde\sigma_{k,n}}, \hat{y}_{\tilde\sigma_{k',n}}, ... \}$ are trained with Cross-Path Consistency Loss described in section ~\ref{section3.3}. }
    \label{fig1}
    % \vspace{-12pt}
\end{figure*}



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Figure_caption/figure1.tex <==
\begin{figure}[tp]
% \centering
\begin{subfigure}[t]{.32\linewidth}
\includegraphics[width=\textwidth]{Figure/cycle.png}
\caption{cycle consistency}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\includegraphics[width=\textwidth]{Figure/task.png}
\caption{cross-task consistency}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\includegraphics[width=\textwidth]{Figure/path.png}
\caption{cross-path consistency}
\end{subfigure}
\caption{\textbf{Comparison on the variants of consistencies}. The black line refers to the main task function $f_{\mathcal{X}\mathcal{Y}}$, and the {\color{red}red}, {\color{blue}blue} lines refer to the pair of tasks trained to be consistent with each other. (a) Cycle consistency enforces the composite function of $f_{\mathcal{Y}\mathcal{X}} \circ f_{\mathcal{X}\mathcal{Y}}$ to be consistent with identity function $f_{\mathcal{X}\mathcal{X}}$. (b) Cross-task consistency requires an auxiliary pretrained network $f_{\mathcal{Y}\mathcal{Y_\text{a}}}$, represented in dashed lines, to give consistent outputs across tasks. (c) Cross-path consistency does not require task-specific pretrained networks. The output of main task function $f_{\mathcal{X}\mathcal{Y}}$ should be consistent with the composition of the outputs from sub-task functions $f_{\mathcal{X}\mathcal{Y_\text{s}}}$ and $f_{\mathcal{Y}_\text{s}\mathcal{Y}} \circ f_{\mathcal{X}\mathcal{Y}_\text{s}}$.}
\label{fig:consistency variants}
\end{figure}


==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Figure_caption/pathnum_ablation.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[t]{0.49\linewidth}
\includegraphics[width=\textwidth]{Figure/ablation_QPIC.png}
\caption{QPIC}
\end{subfigure}
\begin{subfigure}[t]{0.49\linewidth}
\includegraphics[width=\textwidth]{Figure/ablation_HOTR.png}
\caption{HOTR}
\end{subfigure}
\caption{\textbf{Ablation on the number of augmented paths}. As the number of augmented paths increases, main task performance increases accordingly.}
% \caption{Ablation on the number of augmented paths. Performance on the four cases of $\paths_1$, $\paths_1 + \paths_2$, $\paths_1 + \paths_2 + \paths_3$, and $\paths_1 + \paths_2 + \paths_3 + \paths_4$ are compared. As the number of augmented paths increases, main task performance increases accordingly.}
\vspace{-14pt}
\label{fig:pathnum ablation}
\end{figure}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/HICO_new.tex <==
\begin{table*}[!ht]
  \centering
  \footnotesize
  \begin{tabular}{l c c c c c c}
    \toprule
    \multicolumn{4}{c}{} & \multicolumn{3}{c}{\textbf{Default}} \\
    \cmidrule(r){5-7}
    Method & \hspace{12pt}Detector\hspace{12pt} & Backbone & \hspace{12pt}Extra\hspace{12pt} & \hspace{12pt}Full\hspace{12pt} & \hspace{6pt}Rare\hspace{6pt} & Non Rare\hspace{6pt} \\ \midrule\midrule
    % \rowcolor[gray]{0.85}\multicolumn{7}{l}{\textit{\textbf{Sequential HOI Detectors (Instance-centric)}}} \\ \hline
    % \multicolumn{5}{l}{\textit{Models \textbf{with} linguistic priors}} \\ \hline
    % \multicolumn{5}{l}{\textit{Models \textbf{without} linguistic priors}} \\ \hline
    % \multicolumn{1}{l|}{VSRL~\cite{gupta2015visual}} & COCO & VGG-19 & \multicolumn{1}{c|}{A+P} & 6.46 & 4.24 & 7.12  \\
    % \multicolumn{1}{l|}{HO-RCNN~\cite{chao2018learning}} & COCO & CaffeNet & \multicolumn{1}{c|}{A+S} & 7.81 & 5.37 & 8.54  \\
     \multicolumn{3}{l}{ {\textbf{CNN-based HOI Detection Model}}} &  &  &  &  \\ \midrule
    \multicolumn{1}{l|}{InteractNet~\cite{gkioxari2018detecting}} & COCO & R50-FPN & \multicolumn{1}{c|}{\xmark} & 9.94 & 7.16 & 10.77  \\
    % \multicolumn{1}{l|}{Verb Embedding~\cite{xu2019learning}} & COCO & R50 & \multicolumn{1}{c|}{A+L} & 14.70 & 13.26 & 15.13  \\
    \multicolumn{1}{l|}{iCAN~\cite{gao2018ican}} & COCO & R50 & \multicolumn{1}{c|}{S} & 14.84 & 10.45 & 16.15  \\
    \multicolumn{1}{l|}{TIN~\cite{li2019transferable}} & COCO & R50 & \multicolumn{1}{c|}{S+P} & 17.03 & 13.42 & 18.11  \\
    \multicolumn{1}{l|}{RPNN~\cite{zhou2019relation}} & COCO & R50 & \multicolumn{1}{c|}{P} & 17.35 & 12.78 & 18.71  \\
    \multicolumn{1}{l|}{PMFNet~\cite{wan2019pose}} & COCO & R50-FPN & \multicolumn{1}{c|}{S+P} & 17.46 & 15.65 & 18.00  \\
    \multicolumn{1}{l|}{No-Frills HOI~\cite{gupta2019no}} & COCO & R152 & \multicolumn{1}{c|}{S+P} & 17.18 & 12.17 & 18.68  \\
    % \multicolumn{1}{l|}{Analogies~\cite{peyre2019detecting}} & COCO & R50-FPN & \multicolumn{1}{c|}{A+L} & 19.4 & 14.6 & 20.9  \\
    \multicolumn{1}{l|}{UnionDet~\cite{Kim2020UnionDet}} & COCO & R50-FPN & \multicolumn{1}{c|}{\xmark} & 14.25 & 10.23 & 15.46 \\
    \multicolumn{1}{l|}{DRG~\cite{Gao2020DRG}} & COCO & R50-FPN & \multicolumn{1}{c|}{S+L} & 19.26 & 17.74 & 19.71  \\
    \multicolumn{1}{l|}{VCL~\cite{Hou2020VCL}} & COCO & R50 & \multicolumn{1}{c|}{S} & 19.43 & 16.55 & 20.29  \\
    \multicolumn{1}{l|}{FCMNet~\cite{Liu2020FCMNet}} & COCO & R50 & \multicolumn{1}{c|}{S+P} & 20.41	& 17.34	& 21.56  \\
    \multicolumn{1}{l|}{ACP~\cite{Kim2020ACP}} & COCO & R152 & \multicolumn{1}{c|}{S+P} & 20.59 & 15.92 & 21.98  \\
    \multicolumn{1}{l|}{DJ-RN~\cite{li2020detailed}} & COCO & R50 & \multicolumn{1}{c|}{S+V} & 21.34 & 18.53 & 22.18  \\
    \multicolumn{1}{l|}{ConsNet~\cite{Liu2020ConsNet}} & COCO & R50-FPN & \multicolumn{1}{c|}{S+L} & 22.15 & 17.12 & 23.65  \\
    \multicolumn{1}{l|}{PastaNet~\cite{li2020pastanet}} & COCO & R50 & \multicolumn{1}{c|}{S+P+L} & 22.65 & 21.17 & 23.09  \\
    \multicolumn{1}{l|}{IDN~\cite{yonglu2020idn}} & COCO & R50 & \multicolumn{1}{c|}{S} & 23.36 & 22.47 & 23.63  \\ 
    
    % \rowcolor[gray]{0.85}\multicolumn{7}{l}{\textit{\textbf{Parallel HOI Detectors}}} \\ \hline
    \multicolumn{1}{l|}{GPNN~\cite{qi2018learning}} & COCO & R152 & \multicolumn{1}{c|}{\xmark} & 13.11 & 9.41 & 14.23  \\
    \multicolumn{1}{l|}{IPNet~\cite{wang2020learning}} & COCO & HourGlass104 &\multicolumn{1}{c|}{\xmark} & 19.56 & 12.79 & 21.58 \\
    \multicolumn{1}{l|}{VSGNet~\cite{ulutan2020vsgnet}} & COCO & R152 & \multicolumn{1}{c|}{S} & 19.80 & 16.05 & 20.91  \\
    \multicolumn{1}{l|}{PD-Net~\cite{Xubin2020PDNet}} & COCO & R152 & \multicolumn{1}{c|}{S+P+L} & 20.81 & 15.90 & 22.28  \\ \midrule 
    
     \multicolumn{3}{l}{{ \textbf{Transformer-based HOI Detection Model}}} &  &  &  &   \\ \midrule
    \multicolumn{1}{l|}{HoiT~\cite{zou2021end}} & HICO-DET & R50 & \multicolumn{1}{c|}{\xmark} & 23.46 & 16.91 & 25.41 \\
    \multicolumn{1}{l|}{AS-Net~\cite{chen2021reformulating}} & HICO-DET & R50 & \multicolumn{1}{c|}{\xmark} & 28.87 & 24.25 & 30.25 \\
     \hline 
    \multicolumn{1}{l|}{HOTR~\cite{kim2021hotr}} & HICO-DET & R50 & \multicolumn{1}{c|}{\xmark} & 25.10 & 17.34 & \textbf{27.42} \\
    \multicolumn{1}{l|}{HOTR+ \textbf{Ours}} & HICO-DET & R50 & \multicolumn{1}{c|}{\xmark} & \textbf{26.16} & \textbf{22.84} & 27.15 \\
    \multicolumn{1}{l|}{QPIC~\cite{tamura2021qpic}} & HICO-DET & R50 & \multicolumn{1}{c|}{\xmark} & 29.07 & 21.85 & 31.23 \\
    \multicolumn{1}{l|}{QPIC+ \textbf{Ours}} & HICO-DET & R50 & \multicolumn{1}{c|}{\xmark} & \textbf{29.63} & \textbf{23.14} & \textbf{31.57} \\
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Performance comparison in HICO-DET}. For the Detector, COCO means that the detector is trained on COCO, while HICO-DET means that the detector is first trained on COCO and then fine-tuned on HICO-DET.  The each letter in Extra column stands for S: Interaction Patterns (Spatial Correlations), P: Pose, L: Linguistic Priors, V: Volume.}
  \label{tab:HICO-DET}
\end{table*}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/Hico.tex <==
\begin{table*}[h!]
  \centering
  \footnotesize
  \begin{tabular}{l c c c c c c}
    \toprule
    \multicolumn{4}{c}{} & \multicolumn{3}{c}{\textbf{Default}} \\
    \cmidrule(r){5-7}
    Method & \hspace{12pt}Detector\hspace{12pt} & Backbone & \hspace{12pt}Extra\hspace{12pt} & \hspace{12pt}Full\hspace{12pt} & \hspace{6pt}Rare\hspace{6pt} & Non Rare\hspace{6pt} \\ \hline 
    % \rowcolor[gray]{0.85}\multicolumn{7}{l}{\textit{\textbf{Sequential HOI Detectors (Instance-centric)}}} \\ \hline
    % \multicolumn{5}{l}{\textit{Models \textbf{with} linguistic priors}} \\ \hline
    % \multicolumn{5}{l}{\textit{Models \textbf{without} linguistic priors}} \\ \hline
    % \multicolumn{1}{l|}{VSRL~\cite{gupta2015visual}} & COCO & VGG-19 & \multicolumn{1}{c|}{A+P} & 6.46 & 4.24 & 7.12  \\
    % \multicolumn{1}{l|}{HO-RCNN~\cite{chao2018learning}} & COCO & CaffeNet & \multicolumn{1}{c|}{A+S} & 7.81 & 5.37 & 8.54  \\
     \multicolumn{3}{l}{ \textit{\textbf{CNN-based HOI Detection Model}}} &  &  &  &  \\ \hline
    \multicolumn{1}{l|}{InteractNet~\cite{gkioxari2018detecting}} & COCO & R50-FPN & \multicolumn{1}{c|}{A} & 9.94 & 7.16 & 10.77  \\
    % \multicolumn{1}{l|}{Verb Embedding~\cite{xu2019learning}} & COCO & R50 & \multicolumn{1}{c|}{A+L} & 14.70 & 13.26 & 15.13  \\
    \multicolumn{1}{l|}{iCAN~\cite{gao2018ican}} & COCO & R50 & \multicolumn{1}{c|}{A+S} & 14.84 & 10.45 & 16.15  \\
    \multicolumn{1}{l|}{TIN~\cite{li2019transferable}} & COCO & R50 & \multicolumn{1}{c|}{A+S+P} & 17.03 & 13.42 & 18.11  \\
    \multicolumn{1}{l|}{RPNN~\cite{zhou2019relation}} & COCO & R50 & \multicolumn{1}{c|}{A+P} & 17.35 & 12.78 & 18.71  \\
    \multicolumn{1}{l|}{PMFNet~\cite{wan2019pose}} & COCO & R50-FPN & \multicolumn{1}{c|}{A+S+P} & 17.46 & 15.65 & 18.00  \\
    \multicolumn{1}{l|}{No-Frills HOI~\cite{gupta2019no}} & COCO & R152 & \multicolumn{1}{c|}{A+S+P} & 17.18 & 12.17 & 18.68  \\
    % \multicolumn{1}{l|}{Analogies~\cite{peyre2019detecting}} & COCO & R50-FPN & \multicolumn{1}{c|}{A+L} & 19.4 & 14.6 & 20.9  \\
    \multicolumn{1}{l|}{UnionDet~\cite{Kim2020UnionDet}} & COCO & R50-FPN & \multicolumn{1}{c|}{A} & 14.25 & 10.23 & 15.46 \\
    \multicolumn{1}{l|}{DRG~\cite{Gao2020DRG}} & COCO & R50-FPN & \multicolumn{1}{c|}{A+S+L} & 19.26 & 17.74 & 19.71  \\
    \multicolumn{1}{l|}{VCL~\cite{Hou2020VCL}} & COCO & R50 & \multicolumn{1}{c|}{A+S} & 19.43 & 16.55 & 20.29  \\
    \multicolumn{1}{l|}{FCMNet~\cite{Liu2020FCMNet}} & COCO & R50 & \multicolumn{1}{c|}{A+S+P} & 20.41	& 17.34	& 21.56  \\
    \multicolumn{1}{l|}{ACP~\cite{Kim2020ACP}} & COCO & R152 & \multicolumn{1}{c|}{A+S+P} & 20.59 & 15.92 & 21.98  \\
    \multicolumn{1}{l|}{DJ-RN~\cite{li2020detailed}} & COCO & R50 & \multicolumn{1}{c|}{A+S+V} & 21.34 & 18.53 & 22.18  \\
    \multicolumn{1}{l|}{ConsNet~\cite{Liu2020ConsNet}} & COCO & R50-FPN & \multicolumn{1}{c|}{A+S+L} & 22.15 & 17.12 & 23.65  \\
    \multicolumn{1}{l|}{PastaNet~\cite{li2020pastanet}} & COCO & R50 & \multicolumn{1}{c|}{A+S+P+L} & 22.65 & 21.17 & 23.09  \\
    \multicolumn{1}{l|}{IDN~\cite{yonglu2020idn}} & COCO & R50 & \multicolumn{1}{c|}{A+S} & 23.36 & 22.47 & 23.63  \\ 
    
    % \rowcolor[gray]{0.85}\multicolumn{7}{l}{\textit{\textbf{Parallel HOI Detectors}}} \\ \hline
    \multicolumn{1}{l|}{GPNN~\cite{qi2018learning}} & COCO & R152 & \multicolumn{1}{c|}{A} & 13.11 & 9.41 & 14.23  \\
    \multicolumn{1}{l|}{IPNet~\cite{wang2020learning}} & COCO & HourGlass104 & \multicolumn{1}{c|}{A} & 19.56 & 12.79 & 21.58 \\
    \multicolumn{1}{l|}{VSGNet~\cite{ulutan2020vsgnet}} & COCO & R152 & \multicolumn{1}{c|}{A+S} & 19.80 & 16.05 & 20.91  \\
    \multicolumn{1}{l|}{PD-Net~\cite{Xubin2020PDNet}} & COCO & R152 & \multicolumn{1}{c|}{A+S+P+L} & 20.81 & 15.90 & 22.28  \\ \hline 
    
    \rowcolor{Gray} \multicolumn{3}{l}{\textit{ \textbf{Transformer-based HOI Detection Model}}} &  &  &  &   \\ \hline
    \multicolumn{1}{l|}{HoiT~\cite{zou2021end}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & 23.46 & 16.91 & 25.41 \\
    \multicolumn{1}{l|}{AS-Net~\cite{chen2021reformulating}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & 28.87 & 24.25 & 30.25 \\
    \multicolumn{1}{l|}{CDN~\cite{zhang2021mining}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & \textbf{31.78} & \textbf{27.55} & \textbf{33.05} \\ \hline 
    \multicolumn{1}{l|}{HOTR~\cite{kim2021hotr}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & 25.10 & 17.34 & \textbf{27.42} \\
    \multicolumn{1}{l|}{HOTR+ \textbf{Ours}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & \textbf{26.16} & \textbf{22.84} & 27.15 \\
    \multicolumn{1}{l|}{QPIC~\cite{tamura2021qpic}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & 29.07 & 21.85 & 31.23 \\
    \multicolumn{1}{l|}{QPIC+ \textbf{Ours}} & HICO-DET & R50 & \multicolumn{1}{c|}{A} & \textbf{29.63} & \textbf{23.14} & \textbf{31.57} \\
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Performance comparison in HICO-DET}. For the Detector, COCO means that the detector is trained on COCO, while HICO-DET means that the detector is first trained on COCO and then fine-tuned on HICO-DET.  The each letter in Feature column stands for A: Appearance, S: Interaction Patterns (Spatial Correlations), P: Pose, L: Linguistic Priors, V: Volume.}
  \label{tab:HICO-DET role}
\end{table*}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/Vcoco.tex <==
\begin{table}[ht]
  \centering
  \footnotesize
  \begin{tabular}{l|c|c c}
    \toprule
    Method\hspace{15pt} & \hspace{15pt}Backbone\hspace{15pt} & \scone & 
    \sctwo  \\ \midrule \midrule
     \multicolumn{4}{l}{ {\textbf{CNN-based HOI Detection Model}}}\vspace{0.3pt} \\ \midrule
    % VSRL~\cite{gupta2015visual} & R50-FPN  & 31.8 & - \\
    InteractNet~\cite{gkioxari2018detecting} & R50-FPN & 40.0 & 48.0 \\
    % BAR-CNN~\cite{kolesnikov2018detecting} & R50-FPN  & 43.6 & - \\
    iCAN~\cite{gao2018ican} & R50 & 45.3 & 52.4 \\
    TIN~\cite{li2019transferable} & R50  & 47.8 & - \\
    RPNN~\cite{zhou2019relation} & R50  & - & 47.5 \\
    Verb Embd.~\cite{xu2019learning} & R50 & 45.9 & - \\
    PMFNet~\cite{wan2019pose} & R50-FPN  & 52.0 & - \\
    PastaNet~\cite{li2020pastanet} & R50-FPN  & 51.0 & 57.5 \\ 
    % Cascaded~\cite{zhou2020cascaded} & R50  & 48.6 & - \\
    VCL~\cite{Hou2020VCL}  & R50 L & 48.3 & - \\
    UniDet~\cite{Kim2020UnionDet} & R50-FPN  & 47.5 & 56.2 \\ 
    DRG~\cite{Gao2020DRG} & R50-FPN  & 51.4 & - \\
    % PMN~\cite{Zhijun2020pmn} & R50-FPN  & 51.8 & - \\ 
    % Hetero~\cite{Wang2020Hetero} & R50-FPN  & 52.7 & - \\
    FCMNet~\cite{Liu2020FCMNet} & R50  & 53.1 & - \\
    ConsNet~\cite{Liu2020ConsNet} & R50-FPN  & 53.2 & - \\
    PDNet~\cite{Xubin2020PDNet} & R50-FPN  & 53.3 & - \\
    IDN~\cite{yonglu2020idn} & R50  & 53.3 & 60.3 \\ 
    GPNN~\cite{qi2018learning} & R152 & 44.0 & - \\
    IPNet~\cite{wang2020learning} & H.G.104 & 51.0 & - \\
    VSGNet~\cite{ulutan2020vsgnet} & R152  & 51.8 & 57.0 \\ 
    PDNet~\cite{Xubin2020PDNet}  & Res152  & 52.2 & - \\ 
    ACP~\cite{Kim2020ACP} & Res152  & 53.0 & - \\  \midrule
     \multicolumn{4}{l}{ {\textbf{Transformer-based HOI Detection Model}}}  \\  \midrule 
    HoiT ~\cite{zou2021end} & R101  & 52.9 & - \\
    AS-Net ~\cite{chen2021reformulating} & R50  & 53.9 & - \\
   
    \hline
    HOTR ~\cite{kim2021hotr} & R50  & 55.2 & 64.4 \\
    HOTR+ \textbf{Ours} & R50 & \textbf{61.6} & \textbf{66.8}  \\
    QPIC ~\cite{tamura2021qpic} & R50  & 58.8 & 61.0 \\
    QPIC+ \textbf{Ours} & R50 & \textbf{63.1} &\textbf{ 65.4} \\
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \caption{\textbf{Comparison of performances on the V-COCO test set}. {AP}${}^{}_{\text{role1}}$  and {AP}${}^{}_{\text{role2}}$ denotes performances under Scenario 1 and Scenario 2 in V-COCO respectively.} 
  \label{tab:V-COCO}
\end{table}

% \begin{table*}[h!]
%   \centering
%   \footnotesize
%   \begin{tabular}{l|c|c|c c}
%     \toprule
%     Method\hspace{70pt} & \hspace{15pt}Backbone\hspace{15pt} & \hspace{15pt}Features\hspace{15pt} & mAP(Sc.\#1) & mAP(Sc.\#2) \\ \midrule
%     VSRL~\cite{gupta2015visual} & R50-FPN & A & 31.8 & - \\
%     InteractNet~\cite{gkioxari2018detecting} & R50-FPN & A & 40.0 & 47.98 \\
%     BAR-CNN~\cite{kolesnikov2018detecting} & R50-FPN & A+S & 43.6 & - \\
%     iCAN~\cite{gao2018ican} & R50 & A+S & 45.3 & 52.4 \\
%     TIN~\cite{li2019transferable} & R50 & A+S+P & 47.8 & - \\
%     RPNN~\cite{zhou2019relation} & R50 & A+P & - & 47.5 \\
%     Verb Embd.~\cite{xu2019learning} & R50 & A+L & 45.9 & - \\
%     PMFNet~\cite{wan2019pose} & R50-FPN & A+S+P & 52.0 & - \\
%     PastaNet~\cite{li2020pastanet} & R50-FPN & A+P+L & 51.0 & 57.5 \\ 
%     Cascaded~\cite{zhou2020cascaded} & R50 & A & 48.6 & - \\
%     VCL~\cite{Hou2020VCL}  & R50 & A+L & 48.3 & - \\
%     UniDet~\cite{Kim2020UnionDet} & R50-FPN & A & 47.5 & 56.2 \\ 
%     DRG~\cite{Gao2020DRG} & R50-FPN & A+S+L & 51.37 & - \\
%     PMN~\cite{Zhijun2020pmn} & R50-FPN & A+S+P & 51.8 & - \\ 
%     Hetero~\cite{Wang2020Hetero} & R50-FPN & A & 52.7 & - \\
%     FCMNet~\cite{Liu2020FCMNet} & R50 & A+S+P & 53.1 & - \\
%     ConsNet~\cite{Liu2020ConsNet} & R50-FPN & A+L & 53.2 & - \\
%     PDNet~\cite{Xubin2020PDNet} & R50-FPN & A+S+L+P & 53.3 & - \\
%     IDN~\cite{yonglu2020idn} & R50 & A+S+L+P & 53.3 & 60.3 \\ 
%     GPNN~\cite{qi2018learning} & R152 & A & 44.0 & - \\
%     IPNet~\cite{wang2020learning} & HourGlass104 & A & 51.0 & - \\
%     VSGNet~\cite{ulutan2020vsgnet} & R152 & A+S & 51.76 & 57.03 \\ 
%     PDNet~\cite{Xubin2020PDNet}  & Res152 & A+S+L & 52.2 & - \\ 
%     ACP~\cite{Kim2020ACP} & Res152 & A+P+L & 52.98 & - \\  \midrule
%     HOTR ~\cite{kim2021hotr} & R50 & A & 55.2 & 64.4 \\
%     QPIC ~\cite{tamura2021qpic} & R50 & A & 58.8 & 61.0 \\
%     HoiT ~\cite{zou2021end} & R101 & A & 52.9 & - \\
%     AS-Net ~\cite{chen2021reformulating} & R50 & A & 53.9 & - \\
%     CDN~\cite{zhang2021mining} & R50 & A & 62.29 & 64.42 \\
%     \midrule
%     \textit{\textbf{Ours}} & R50 & A & - & - \\
%     \bottomrule
%   \end{tabular}
%   \vspace{5pt}
%   \caption{Comparison of performance on V-COCO test set. The each letter in Feature column stands for A: Appearance, S: Interaction Patterns (Spatial Correlations), P: Pose, L: Linguistic Priors, V: Volume.} 
%   \label{tab:V-COCO role}
% \end{table*}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/ablation1_pathwise_seperate.tex <==
\begin{table}[h]
    \centering
    % \caption{Ablation.}
    % \footnotesize
    \small
    \begin{tabular}{c c c c c c}
         \toprule
         \multirow{1}{*}{\textbf{Method}} &  \multicolumn{1}{c}{$\paths_1$}
         &\multicolumn{1}{c}{$\paths_2$}
         &\multicolumn{1}{c}{$\paths_3$}
         &\multicolumn{1}{c}{$\paths_4$}
         &\multicolumn{1}{c}{\textbf{\textit{Average}}} \\
         
         \midrule    
         \midrule
         
         \multirow{1}{*}{QPIC} &
         62.2 & 
         61.9 &
         61.7 &
         60.4 &
         61.55 $\pm$ 0.69 
         \\
         
         \midrule
        
         \multirow{1}{*}{HOTR}&
         59.8 &  
         59.5 & 
         59.0 & 
         58.9 & 
         59.3 $\pm$ 0.37  
         \\
        
         
         \bottomrule
    \end{tabular}
    \caption{
    % Path-wise and average results on V-COCO. 
    \textbf{Path-wise results on V-COCO.}
    }
    \label{table:abl_pathwise_sep}
\end{table}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/ablation_pathnum.tex <==
\begin{table*}[h]
    \centering
    \footnotesize
    \begin{tabular}{c  c c   c c   c c   c c}
         \toprule
         \multirow{3}{*}{\textbf{Method}} 
         &\multicolumn{2}{c}{$\paths_1$}
         &\multicolumn{2}{c}{$\paths_1+\paths_2$}
         &\multicolumn{2}{c}{$\paths_1+\paths_2+\paths_3$}
         &\multicolumn{2}{c}{$\paths_1+\paths_2+\paths_3+\paths_4$} \\
         
         \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
        & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo 
        \\ 
  
         \midrule
         
         \multirow{1}{*}{QPIC} &
         62.16 & 64.53 & 
             &   &
             &   &
             &   
         \\
         \midrule
        
         \multirow{1}{*}{HOTR} &
         59.83 & 64.90 &
         60.94 & 66.10 &
         61.42 & 66.77 &
         \textbf{61.60} & \textbf{66.84} 
         \\
         \bottomrule
    \end{tabular}
    \caption{Ablation Study on the number of augmented paths in V-COCO.}
    \label{table:abl_num}
\end{table*}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/ablation_pathnum_noS2.tex <==
\begin{table}[h]
    \centering
   
    \footnotesize
    \begin{tabular}{c c c c c}
         \toprule
         \multirow{1}{*}{\textbf{Number of Paths}} 
         &\multicolumn{1}{c}{1}
         &\multicolumn{1}{c}{2}
         &\multicolumn{1}{c}{3}
         &\multicolumn{1}{c}{4} \\
        %  &\multicolumn{1}{c}{\hspace*{10mm}$\paths_1$\hspace*{10mm}}
        %  &\multicolumn{1}{c}{\hspace*{6mm}$\paths_1+\paths_2$\hspace*{6mm}}
        %  &\multicolumn{1}{c}{\hspace*{2mm}$\paths_1+\paths_2+\paths_3$\hspace*{2mm}}
        %  &\multicolumn{1}{c}{$\paths_1+\paths_2+\paths_3+\paths_4$} \\
         
  
         \midrule
         
         \multirow{1}{*}{QPIC} &
         62.16 & 
         62.57&   
         62.71&  
         \textbf{63.11}
         \\
         \midrule
        
         \multirow{1}{*}{HOTR} &
         59.83 &  
         60.94 & 
         61.42 & 
         \textbf{61.60}  
         \\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation on the number of augmented paths}. Performance on the four cases of $\paths_1$, $\paths_1 + \paths_2$, $\paths_1 + \paths_2 + \paths_3$, and $\paths_1 + \paths_2 + \paths_3 + \paths_4$ are compared.}
    \label{table:abl_num}
\end{table}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/ablation_pathwise.tex <==
\begin{table*}[h]
    \centering
    % \caption{Ablation.}
    \footnotesize
    \begin{tabular}{c c c  c c   c c   c c   c c   c c}
         \toprule
         \multirow{3}{*}{\textbf{Method}} & 
         \multirow{3}{*}{\textit{Share Dec.}} &
         \multirow{3}{*}{$\  $\textit{CPC}$\  $}& \multicolumn{2}{c}{$\paths_1$}
         &\multicolumn{2}{c}{$\paths_2$}
         &\multicolumn{2}{c}{$\paths_3$}
         &\multicolumn{2}{c}{$\paths_4$}
         &\multicolumn{2}{c}{\textbf{\textit{Average}}} \\
         
         \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13} 
        &  &  & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo & 
        \scone & 
        \sctwo  
        \\ 
  
         \midrule
         
         \multirow{3}{*}{QPIC} & & &
         62.16 & 64.53 & 
         61.89 & 64.13 &
         61.73 & 64.17 &
         60.43 & 62.95 &
         61.55 $\pm$ 0.66 &
         63.95 $\pm$ 0.60
         \\
         & \checkmark& & 
         60.65 & 63.16 & 
         60.69 & 63.21 &
         59.88 & 62.26 & 
         58.10 & 60.37 & 
         59.83 $\pm$ 1.04 &
         62.25 $\pm$ 1.15
         \\
         & \checkmark&\checkmark & 
         \textbf{63.11} & \textbf{65.44} & 
         \textbf{63.31} & \textbf{65.84} &
         \textbf{63.12} & \textbf{65.40} &
         \textbf{63.01} & \textbf{65.30} &
         \textbf{63.18} $\pm$ 0.10${}^\dagger$ &
         \textbf{65.45} $\pm$ 0.20${}^\dagger$ \\
         \midrule
        
         \multirow{3}{*}{HOTR} & & &
         59.83 & 64.90 &
         59.49 & 64.28 &
         58.98 & 64.13 &
         58.90 & 63.82 &
         59.30 $\pm$ 0.48 & 
         64.28 $\pm$ 0.39
         \\
         & \checkmark& & 
         60.61 & 65.39 &
         60.63 & 65.35 &
         61.17 & 66.01 &
         60.61 & 65.67 & 
         60.75 $\pm$ 0.24 & 
         65.58 $\pm$ 0.26
         \\
         & \checkmark&\checkmark &
         \textbf{61.60} & \textbf{66.84} & 
         \textbf{61.48} & \textbf{66.70} &
         \textbf{61.58} & \textbf{66.76} &
         \textbf{61.63} & \textbf{66.76} &
         \textbf{61.57} $\pm$ 0.05${}^\dagger$ & 
         \textbf{66.76} $\pm$ 0.04${}^\dagger$
         \\
         \bottomrule
    \end{tabular}
    \caption{Ablation Study for path-wise and average results of all paths in V-COCO.}
    \label{table:abl}
\end{table*}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/ablation_pathwise_noS2.tex <==
\begin{table*}[ht]
    \centering
    % \caption{Ablation.}
    % \footnotesize
    \small
    \begin{tabular}{c c c   c c c c c}
         \toprule
         \multirow{1}{*}{\textbf{Method}} & 
         \multirow{1}{*}{\textit{Share Dec.}} &
         \multirow{1}{*}{$\  $\textit{CPC}$\  $}& \multicolumn{1}{c}{$\paths_1$}
         &\multicolumn{1}{c}{$\paths_2$}
         &\multicolumn{1}{c}{$\paths_3$}
         &\multicolumn{1}{c}{$\paths_4$}
         &\multicolumn{1}{c}{\textbf{\textit{Average}}} \\
         
         \midrule    
         \midrule
         
         \multirow{3}{*}{QPIC} 
         
         & \checkmark
         &\checkmark & 
         \textbf{63.1} & 
         \textbf{63.3} &  
         \textbf{63.1} & 
         \textbf{63.0} & 
         \textbf{63.13} $\pm$ 0.05${}^\dagger$ \\
         
         & 
         &\checkmark & 
         62.4 & 
         62.9 &  
         60.8 & 
         59.4 & 
         61.38 $\pm$ 1.38 \\
         
         & \checkmark
         &  &
         60.7 &
         60.7 &
         59.9 & 
         58.1 &
         59.85 $\pm$ 1.06 
         \\
         
         \midrule
         
         
        
         \multirow{3}{*}{HOTR} 
         
         & \checkmark
         &\checkmark &
         \textbf{61.6} &  
         61.5 & 
         \textbf{61.6} &  
         \textbf{61.6} &  
         \textbf{61.58} $\pm$ 0.02${}^\dagger$  
         \\
         
         & 
         &\checkmark &
         61.2 &  
         \textbf{61.6} & 
         61.1 &  
         60.6 &  
         61.13 $\pm$ 0.36  
         \\
         
         & \checkmark& & 
         60.6 & 
         60.6 &  
         61.2 &  
         60.6 &  
         60.75 $\pm$ 0.13 
         \\
         
         
         \bottomrule
    \end{tabular}
    \caption{
    % Path-wise and average results on V-COCO. 
    \textbf{Ablation Study on our learning strategies}. Ablation results on shared decoder (\textit{Share Dec.}), and Cross-Path Consistency (CPC) are demonstrated. For main path $\mathcal{P}_1$, and each augmented path $\mathcal{P}_2$, $\mathcal{P}_3$, $\mathcal{P}_4$, their performances are reported measured in mAP. They are evaluated on the V-COCO test set with respect to Scenario 1. The best performances for each path are highlighted in bold, and $\dagger$ refers to the case where the least standard deviation is observed. 
    }
    \label{table:abl}
\end{table*}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/main_short.tex <==

\begin{table}[!ht]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l  c c  c  c c }
         \toprule
         \multicolumn{1}{c}{} &\multicolumn{2}{c}{V-COCO}& \multicolumn{3}{c}{HICO-DET} \\
         \cmidrule(r){2-3}
         \cmidrule(r){4-6}
         Method & 
         \scone & 
         \sctwo & 
         $\  $ {Full} $\  $ & 
         {Rare} & 
         {Non-Rare   }
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        QPIC & 62.2* & 64.5* &29.07 &21.85& 31.23 \\
        QPIC + ours & \textbf{63.1} & \textbf{65.4}& \textbf{29.63}&\textbf{23.14} &\textbf{31.57}  \\
         \midrule
         
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         HOTR& 59.8* & 64.9* & 25.10& 17.34&\textbf{27.42}  \\
         HOTR + ours& \textbf{61.6}&\textbf{66.8} &\textbf{26.16} &\textbf{22.84} &27.15  \\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison of our training strategy with vanilla HOI transformers on V-COCO and HICO-DET}. * signifies our results reproduced with the official implementation codes of QPIC and HOTR.}
    \label{table:comp}
    
\end{table}



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/rebuttal_r1_table_option2.tex <==

\begin{table}[!ht]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l  c c  c  c c }
         \toprule
         \multicolumn{1}{c}{} &\multicolumn{2}{c}{V-COCO}& \multicolumn{3}{c}{HICO-DET} \\
         \cmidrule(r){2-3}
         \cmidrule(r){4-6}
         Method & 
         \scone & 
         \sctwo & 
         $\  $ {Full} $\  $ & 
         {Rare} & 
         {Non-Rare   }
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        QPIC & 58.8 & 61.0 &29.07 &21.85& 31.23 \\
        QPIC + ours & \textbf{63.1} & \textbf{65.4}& \textbf{xx}&\textbf{xx} &\textbf{xx}  \\
         \midrule
         
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         HOTR& 55.2 & 64.4 & 25.10& 17.34&\textbf{27.42}  \\
         HOTR + ours& \textbf{61.6}&\textbf{66.8} &\textbf{xx} &\textbf{xx} &xx \\
         \bottomrule
    \end{tabular}
    \caption{Abstraction of table 2 and table 3 in main paper.}
    \label{table:rebuttal_comp2}
    
\end{table}



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/rebuttal_r1_table_option4.tex <==

\begin{table}[!ht]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l  c c  c  c c }
         \toprule
         \multicolumn{1}{c}{} &\multicolumn{2}{c}{V-COCO}& \multicolumn{3}{c}{HICO-DET} \\
         \cmidrule(r){2-3}
         \cmidrule(r){4-6}
         Method & 
         \scone & 
         \sctwo & 
         $\  $ {Full} $\  $ & 
         {Rare} & 
         {Non-Rare   }
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        QPIC & 62.2* & 64.5* &29.07 &21.85& 31.23 \\
        QPIC + ours & \textbf{63.1} & \textbf{65.4}& \textbf{29.63}&\textbf{23.14} &\textbf{31.57}  \\
         \midrule
         
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         HOTR& 59.8* & 64.9* & 25.10& 17.34&\textbf{27.42}  \\
         HOTR + ours& \textbf{61.6}&\textbf{66.8} &\textbf{26.16} &\textbf{22.84} &27.15  \\
         \bottomrule
    \end{tabular}
    \caption{Table 1 in main paper.}
    \label{table:rebuttal_comp4}
    
\end{table}



==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/rebuttal_r3_qpicfreezeenc.tex <==

\begin{table}[h]
    \centering
    % \caption{Ablation.}
    \footnotesize
    % \small
    \captionsetup{aboveskip=2pt}
    \begin{tabular}{c c  c  c}
         \toprule
          
        %  \multirow{1}{*}{\textit{Freeze Enc.}} &
         \multirow{1}{*}{\textit{Share Dec.}} &
         \multirow{1}{*}{$\  $\textit{CPC}$\  $}& 
         \multirow{1}{*}{\textbf{QPIC} ($\mathcal{P}_1$)} &
        
         \multirow{1}{*}{\textbf{HOTR} ($\mathcal{P}_1$)} 
         
         \\
         
         \midrule    
      
         
      
         
         
         \checkmark &\checkmark &
         \textbf{65.0} \color{blue}(+1.4)&\textbf{61.6 } \color{blue}(+1.8) \\
         
        
          &\checkmark & 
         64.1 \color{blue}(+0.5) & 61.2 \color{blue}(+1.4) \\
         
        
         \checkmark  & &
         64.0 \color{blue}(+0.4)&60.6 \color{blue}(+0.8)
         \\
         
           & &
         63.6 \color{blue}(+0.0)&59.8 \color{blue}(+0.0)
         \\
         
        
         
         \bottomrule
    \end{tabular}
    \caption{
    % Path-wise and average results on V-COCO. 
    Ablations for decoder sharing and CPC in $\mathcal{P}_1$.}
    \label{table:abl_rebuttal}
\end{table}

% \begin{table}[h]
%     \centering
%     % \caption{Ablation.}
%     \footnotesize
%     % \small
%     \begin{tabular}{c  c   c c }
%          \toprule
%          \multirow{1}{*}{\textbf{Method}} & 
%         %  \multirow{1}{*}{\textit{Freeze Enc.}} &
%          \multirow{1}{*}{\textit{Share Dec.}} &
%          \multirow{1}{*}{$\  $\textit{CPC}$\  $}& \multicolumn{1}{c}{$\paths_1$}
         
%          \\
         
%          \midrule    
%          \midrule
         
%          \multirow{4}{*}{QPIC} 
         
         
%          &\checkmark &\checkmark &
%          \textbf{65.0}  \\
         
        
%          & &\checkmark &
%          64.1  \\
         
        
%          &\checkmark  & &
%          64.0 
%          \\
         
%          &  & &
%          63.6
%          \\
         
%          \midrule
         
         
        
%          \multirow{4}{*}{HOTR} 
         
         
%          &\checkmark & \checkmark&
%          \textbf{61.6} 
%          \\
         
         
%          &&\checkmark  &
%          61.2 
%          \\
         
%          & \checkmark& &
%          60.6 
%          \\
%          & & &
%          59.8 
%          \\
         
         
%          \bottomrule
%     \end{tabular}
%     \caption{
%     % Path-wise and average results on V-COCO. 
%     Ablations for decoder sharing and CPC in $\mathcal{P}_1$.}
%     \label{table:abl_rebuttal}
% \end{table}


==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/supple_asnet.tex <==

\begin{table}[!h]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l c c   c  c c }
         \toprule
         \multicolumn{1}{c}{} &
         \multicolumn{2}{c}{} &
         \multicolumn{3}{c}{HICO-DET} \\

         \cmidrule(r){4-6}
         Method & 
         epoch &
         $\lambda$&
         $\  $ {Full} $\  $ & 
         {Rare} & 
         {Non-Rare   }
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         AS-Net&90&-&28.87& 24.25&30.25\\
         AS-Net + ours&90&0.5&\textbf{29.13}&\textbf{25.18} &\textbf{30.31}  \\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison of our training strategy with AS-Net on HICO-DET}. 
    }
    \label{table:supple_asnet}
    
\end{table}


==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/supple_coef_hotr.tex <==
\begin{table}[!h]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l  c c  c }
         \toprule

    
         Dataset 
         & epoch
         & $\lambda$ 
         & $t_\text{max}$
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        V-COCO 
        & 90
        & 1
        & 30\\
       
         \midrule
         
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         HICO-DET
        & 50
        & 0.2
        & 20\\
         \bottomrule
    \end{tabular}
    %\caption{\textbf{Hyperparameters for the weight scheduler for HOTR}}
    % \caption{\textbf{Weight scheduler for total CPC loss for HOTR}}
    \caption{\textbf{Weight scheduler settings for HOTR}}
    % \caption{\textbf{Total CPC loss coefficient for HOTR}}
    \label{table:hotr-coef}
    
\end{table}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/supple_coef_qpic.tex <==
\begin{table}[!h]
    \centering
    \footnotesize
    % \caption{Ablation.}

    \begin{tabular}{l  c c  c }
         \toprule

    
         Dataset 
         &epoch
         & $\lambda$ 
         & $t_\text{max}$
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        V-COCO 
        & 90
        & 0.2
        & 30\\
       
         \midrule
         
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
         HICO-DET
        & 90
        & 0.2
        & 30\\
         \bottomrule
    \end{tabular}
    %\caption{\textbf{Total CPC loss coefficient for QPIC}}
    \caption{\textbf{Weight scheduler settings for QPIC}}
    \label{table:qpic-coef}
    
\end{table}

==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/Table/supple_hoit.tex <==
% \begin{table}[!h]
%     \centering
%     \footnotesize
%     % \caption{Ablation.}
    
%     \begin{tabular}{l c c   c   }
%          \toprule
%          \multicolumn{1}{c}{} &
%          \multicolumn{2}{c}{} &
%          \multicolumn{3}{c}{V-COCO} \\

%          \cmidrule(r){4}
%          Method & 
%          epoch &
%          $\lambda$&
%          $\scone $ & 
%          \\
%          \midrule
%          \midrule
         
%         %  \rowcolor{Gray} 
%         %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
%         %  \\ \midrule
        
%         %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
%         HoiT & 150 & & 48.75* &  \\
%         HoiT + ours & 150 & 0.2 &49.34& \\
%          \bottomrule
%     \end{tabular}
%     \caption{\textbf{Comparison of our training strategy with HoiT on V-COCO and HICO-DET}. 
%     * signifies our results reproduced with the official implementation codes of ~\cite{HOITR}.}
    
%     \label{table:supple_hoit}
    
% \end{table}

\begin{table}[!h]
    \centering
    \footnotesize
    % \caption{Ablation.}
    
    \begin{tabular}{l c c   l}
         \toprule
         \multicolumn{1}{c}{} &
        %  \multicolumn{2}{c}{} &
         \multicolumn{3}{c}{V-COCO} \\
         \cmidrule(l){2-4}
         Method & 
         epoch &
         $\lambda$&
         \scone 
         \\
         \midrule
         \midrule
         
        %  \rowcolor{Gray} 
        %  \multicolumn{6}{l}{ \text{Single-decoder HOI transformer}}   
        %  \\ \midrule
        
        %  \rowcolor{Gray}\multicolumn{6}{l}{ \text{Two-decoder HOI transformer}}   \\ \midrule
         
          HoiT&150&-&48.75*\\
         HoiT + ours&150&0.2&\textbf{49.34} \\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison of our training strategy with HoiT on V-COCO}. * signifies our results reproduced with the official implementation codes of~\cite{HOITR}. 
    }
    \label{table:supple_hoit}
    
\end{table}


==> [CVPR 2022] Consistency Learning via Decoding Path Augmentationfor Transformers in Human Object Interaction Detection/def.tex <==

% feature
\newcommand{\posE}{\text{p}}
\newcommand{\R}{\mathbb{R}}

% architecture
\newcommand{\enc}{\textbf{enc}}
\newcommand{\dec}{\textbf{dec}}

% notation
\newcommand{\paths}{\mathcal{P}}

% Consistency learning
\newcommand{\perm}{\sigma}
\newcommand{\perminv}{\widetilde{\sigma}}
\newcommand{\feature}{\boldsymbol{F}}

% \DeclareMathOperator*{\argmaxB}{argmax}
\newcommand{\comb}[2]{{}_{#1}\mathrm{C}_{#2}}

\newcommand{\xmark}{\ding{55}}
\newcommand{\scone}{{AP}${}^{}_{\text{role1}}$}
\newcommand{\sctwo}{{AP}${}^{}_{\text{role2}}$}
